Towards Automated Discovery of Asymmetric Mempool DoS in Blockchains

In blockchains, mempool controls transaction flow before consensus, denial of whose service hurts the health and security of blockchain networks. This paper presents MPFUZZ, the first mempool fuzzer to find asymmetric DoS bugs by exploring the space of symbolized mempool states and optimistically estimating the promisingness of an intermediate state in reaching bug oracles. Compared to the baseline blockchain fuzzers, MPFUZZ achieves a > 100x speedup in finding known DETER exploits. Running MPFUZZ on major Ethereum clients leads to discovering new mempool vulnerabilities, which exhibit a wide variety of sophisticated patterns, including stealthy mempool eviction and mempool locking. Rule-based mitigation schemes are proposed against all newly discovered vulnerabilities.

==> sty/common-newdefines.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}

%obsoleted due to reviewer complains definition without number
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}




==> sty/ieeetran/ieee-template/editable/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/titlepage.tex <==
\input{sty/title.tex}
\author{
\ifdefined\TTUT
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\fi
}

\maketitle
\IEEEpeerreviewmaketitle



==> sty/ieeetran/usepackage.tex <==
%using latex.XXX file to cusotmize style
%\usepackage{./sty/ieeetran/latex}



==> sty/llncs2e/titlepage.tex <==
\input{sty/title.tex}
\author{
Kai Li\hspace{0.25cm}
Yuzhe (Richard) Tang\hspace{0.25cm}
Beom Heyn (Ben) Kim$\ ^\dag{}$\hspace{0.25cm}
Jianliang Xu$\ ^\ddag{}$\hspace{0.25cm}\\
\ifdefined\TTUT
\fi
}

\institute{
    \fontsize{10}{10}\selectfont\itshape
    Syracuse University, New York, USA\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag{}$University of Toroto, Ontario, Canada\\
    \fontsize{10}{10}\selectfont\itshape
    $^\ddag{}$Hong Kong Baptist University, Kowloon Tong, Hong Kong 
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/titlepage.tex <==
\input{sty/title.tex}
\author{
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/usepackage.tex <==
\usepackage{etoolbox}
\makeatletter
\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
\makeatother

\usepackage{titlesec}
{\filcenter\normalfont\Large\bfseries}
\titleformat{\chapter}
  {\normalfont\sffamily\LARGE\it}
  {\thechapter.}{10pt}{\LARGE}
\titlespacing*{\chapter}{0pt}{0pt}{0pt}
\titleformat{\section}
  {\normalfont\sffamily\Large\bfseries}
  {\thesection.}{0.3em}{}
\titleformat{\subsection}
  {\normalfont\sffamily\large\it}
  {\thesubsection.}{0.3em}{}





==> sty/sig-alternate/titlepage.tex <==
\input{sty/title.tex}
\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\numberofauthors{4} % if number of authors is bigger than number of \alighauthor used following, a ``addtional author'' section will be shown in the end of the paper.
%note: no empty line!
\author{
\alignauthor
Yuzhe Tang$^\dag$
%\titlenote{Author notes}
\\       \affaddr{Syracuse University}
\\       \affaddr{Syracuse, NY 13244}
\\       \email{$^\dag$ytang100@syr.edu}
\ifdefined\TTUT
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\and
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\fi
}
\date{30 July 1999}
\maketitle



==> sty/sig-alternate/titlepage_sharedAuthorAddr.tex <==
\begin{document}
%
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
%
\linespread{0.9}

% --- Author Metadata here ---
\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\title{
Tang's Template of IEEEtran.cls for Conferences \titlenote{!Eye-catching title for high citation: make it short}
}

\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\numberofauthors{1}
\author{
\alignauthor Yuzhe Tang, Ting Wang and Ling Liu \\
  \affaddr{College of Computing, Georgia Institute of Technology} \\ 
  \affaddr{ Atlanta, GA 30332, USA} \\
  \email{yztang@gatech.edu, \{twang, lingliu\}@cc.gatech.edu}
}
\date{30 July 1999}
\maketitle



==> sty/title.tex <==
\begin{document}
% --- Author Metadata here ---
\title{
Towards a Full Understanding of Ethereum Mempool DoS Security
\\ {\normalsize \it Demo submission \today} 
%Full title:
%Automatic Exploit Generation for Understanding Ethereum Mempool DoS Security
%Protecting Ethereum against Asymmetrical DeniAl of Mempool Service (ADAMS) Attacks\\
\ifdefined\TTTOME
Tang's Paper Template \\ Title to be eye-catching for high citation: \\what's new \\short, \\mention approach (to researcher audience)
\fi
}



==> sty/usenix/titlepage.tex <==
\input{sty/title.tex}

\ifdefined\TTUT
\author{
{\rm Your N.\ Here}\\
Your Institution
\and
{\rm Second Name}\\
Second Institution
% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
} % end author
\fi

\maketitle

% Use the following at camera-ready time to suppress page numbers.
% Comment it out when you first submit the paper for review.
\thispagestyle{empty}





==> sty/usenix/usepackage.tex <==
\usepackage{sty/usenix/usenix,epsfig,endnotes}


==> text/buffer.tex <==
{\color{blue}

\begin{figure}[!tb]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/private-tx.eps}
  \caption{Two transaction routes to reach validators: A public transaction route by propagation to all validators and a private transaction route to participating validators without propagation (in green box).}
  \label{fig:eth2:tworoutes}
  \end{figure}

\noindent{\bf Transaction routes before block validation}: On Ethereum 2.0, transactions follow two major routes as illustrated in Figure~\ref{fig:eth2:tworoutes}, to reach a validator node before being included in a block. The first route is public transaction propagation where a transaction is first propagated to reach the entire blockchain network before the current validator node packs it in the next block. Mempool buffers public transactions on this route.

The second route is private transactions. In the most basic form, a private transaction is directly sent to the validator of user's choice without propagation to other nodes. A private transaction can be sent by the user directly, an MEV searcher (reading transactions from mempool), or other causes. In flashbots or PBS, the private transaction is routed to limited nodes in the network, such as relays and proposers. 

Public transactions are buffered in the mempool which is of limited capacity, such as $6144$ transactions by Geth. Private transactions, by contrast, are buffered on the private pool which does not propagate transactions and has a very large (essentially unlimited) capacity. The limited capacity of mempool is necessary; otherwise the number of public transactions per node would grow linearly with the network size (i.e., $O(n)$), exhausting node storage in large networks.
}

===

Given a transaction workload, whether sender accounts are malicious is not observable. As shown in Figure~\ref{fig:example:mitigate:td:ld}, there can be different possibilities. Case 1) accounts $A^1$/$A^2$/$A^3$/$A^4$/$A^5$ are all malicious. Case 2) accounts $A^1$ is malicious. $A^2$/$A^3$/$A^4$/$A^5$ are benign users. Case 3) $A^1$/$A^2$/$A^4$ are malicious. $A^3$/$A^5$ are benign users. In each case, the attacker(s) can mount different attacks, including locking, turning, eviction, etc.

Now consider that the mempool exercises Policy $mp_0$ that admits/evicts transactions by fees. The mempool would admit $A^2_1E^3$ and evict $tx_{A1}$. In Case 1)  (accounts $A^1$/$A^2$/$A^3$/$A^4$/$A^5$ are all malicious), the attackers can successfully mount a turning attack, because evicting $tx_{A1}$ turns $tx_{A2}$ and $tx_{A3}$ into future transactions, reducing the attackers' cost down to zero. Policy $mp_0$ is insecure against TD1, as in Figure~\ref{fig:example:mitigate:td:ld}.

Consider the mempool constrains the transaction admission by Policy $Py_{11}$ (no eviction of parent transactions). Upon the arrival of $A^2_1E^3$, the mempool declines $A^2_1E^3$ as $tx_{A1}$ and $tx_{A2}$ are parents, and $tx_{A3}$ has a higher fee than $t_{B1}$. Similarly, $A^3_1E^5/A^4_1E^3/A^6_1E^5$ are declined. In Case 2) (malicious $A^1$ and benign $A^2$/$A^3$/$A^4$/$A^5$), this is a successful locking attack, as both $A^2_1E^3$ and $A^3_1E^5$ are declined. Policy $Py_{11}$ is insecure under the locking attack, as in Figure~\ref{fig:example:mitigate:td:ld}. 

===

XXX \noindent{\bf Policy $Py_{11}$}: Given an incoming transaction $tx_1$, the mempool finds the residential transaction $tx_2$ that has no further child and has the lowest fee among all residential transactions in the mempool of no children. If $tx_1$'s fee is higher than $tx_2$'s, the mempool admits $tx_1$ by evicting $tx_2$. In other words, the eviction candidate $tx_2$ cannot be a parent transaction.


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Techniques for fuzzing blockchain systems: existing works and mpfuzz's distinction: \xmark{} refers to fuzzing by fixed or random value. \cmark{} refers to fuzzing with semantic awareness.}
\label{tab:rw}\centering{\small
\begin{tabularx}{0.775\textwidth}{ |l|X|c|c|c|c|X| }
  \hline
& Test oracle & \multicolumn{4}{l|}{Tx mutation} & Feedback \\ \cline{3-6}
& & nounce & amount & price & data & \\ \hline
Fluffy~\cite{DBLP:conf/osdi/YangKC21} & EVM-state difference across clients  & \xmark & \xmark & \xmark & \cmark & Code coverage in EVM  \\ \hline
Loki~\cite{DBLP:conf/ndss/MaCRZ00L023} & System crashes & \xmark & \xmark & \xmark & NA & State coverage (msgs) \\ \hline
Tyr~\cite{me:tyr} & Property violation & \xmark & \cmark & \xmark & NA & State divergence + code coverage \\ \hline
mpfuzz & ADAMS & \cmark & \cmark & \cmark & NA & Symbolic state coverage + promisingness \\ \hline
\end{tabularx}
}
\end{table*}



\section{Yibo's Results: Attacking Single Node}

\section{Introduction}

In a public blockchain, anyone on the Internet can join the system and submit transactions. A malicious client can abuse the power and send a flood of transactions to cause denial of service (DoS). While blockchain consensus limits the rate of {\it confirmed} transactions included in the blockchain and prevents the denial of post-consensus services~\cite{nakamoto2009bitcoin,dblp:books/daglib/0040621,dblp:conf/crypto/kiayiasrdo17,dblp:conf/ndss/0002l20,dblp:conf/ispec/chenlwcllaz17}, no effective mechanism exists to limit the rate of {\it unconfirmed} transactions prior to consensus. 
This leaves the DoS of pre-consensus services in an operational blockchain a particularly attractive target for exploitation in practice.

A notable pre-consensus service is buffering unconfirmed transactions on each blockchain node in a cache called mempool. 
The mempool service is critical to the well functioning of the overall blockchain network: 
A disabled mempool can cascade the damage to various downstream services (e.g., mining and transaction propagation) and cause global network disruption. For instance, as demonstrated in a recent study~\cite{DBLP:conf/ccs/LiWT21}, denying the service of top miner nodes' mempools in Ethereum can force the blockchain to produce empty blocks. 

While one can send spamming transactions at high fees to evict normal transactions in a mempool and deny its service, this baseline attack~\cite{DBLP:conf/fc/BaqerHMW16} isn't very practical due to its high cost (e.g., more than 5,000 USD to empty every single Ethereum block).
What poses a more realistic threat is the Asymmetrical DeniAl of Mempool Service, a notion we coin as ADAMS. In ADAMS's threat model, an attacker node sends crafted transactions to one or more selected victim nodes, intending to deny their mempool service at an {\it asymmetrically low cost}. That is, the attacker can cause much more damage (e.g., measured by the fees of evicted victim transactions) than her invested momentary cost (i.e., the fees of crafted transactions).

In the existing literature, DETER~\cite{DBLP:conf/ccs/LiWT21} shows one design pattern of achieving ADAMS, in which the attacker evicts a victim mempool by crafting high-fee but invalid transactions, such as future transactions and latent overdrafts. However, DETER attacks are manually discovered. More importantly, they do not fully explore the input space of transactions when designing attacks. For instance, DETER attacks don't capture certain inter-transaction dependencies such as transaction replacement or take into account more complex cases where a crafted transaction can evict another crafted transaction, recursively. It remains an open question whether there are transaction-crafting patterns other than DETER to cause ADAMS?

{\color{blue}
\noindent{\bf 
Automatic vulnerability discovery}: 
There is a small body of recent works on fuzzing blockchain systems to find consensus failure bugs. {\color{green}{Table~\ref{tab:rw} shows the comparison among these techniques with our work.}} \yw{Table 1 is not referenced} Fluffy~\cite{DBLP:conf/osdi/YangKC21} is a code-coverage-based differential fuzzer to find consensus bugs in Ethereum Virtual Machines (EVM).
%
Loki~\cite{DBLP:conf/ndss/MaCRZ00L023} is a stateful fuzzer to find consensus bugs causing crashes in blockchain network stacks.
%
Tyr~\cite{me:tyr} is a property-based stateful fuzzer that finds consensus bugs causing violations of safety, liveness, integrity, and other properties in blockchain network stacks.
%
However, the existing fuzzing techniques~\cite{me:tyr,DBLP:conf/ndss/MaCRZ00L023,DBLP:conf/osdi/YangKC21} cannot detect mempool DoS bugs, like DETER attacks~\cite{DBLP:conf/ccs/LiWT21}. Briefly, mempool DoS does not trigger a crash (undetected by Loki). Mempool content difference across nodes does not mean insecurity (unlike consensus state difference as detected by Fluffy). 
While Tyr aims to detect liveness and safety violations, its model of invalid transactions is rudimentary. Specifically, they only model double-spending transactions and cannot detect DETER attacks~\cite{DBLP:conf/ccs/LiWT21} that rely on more advanced invalid transactions, like future transactions and latent overdrafts.
}

In this work, we propose automatically discovering ADAMS vulnerabilities and generating exploits against mempool implementations in Ethereum clients.  We formulate it as a stateful fuzzing problem where the test oracle dictates ADAMS conditions on a mempool state. In particular, our fuzzer takes non-code-coverage feedback; the observation is that an ADAMS-satisfying mempool can be reached by running the same code path repeatedly, in other words, without necessarily increasing the code coverage and thus invalidating the existing code-coverage based fuzzer. To guide the input fuzzing, we use as the feedback the ``distance'' between the current mempool state and the destination one that meets ADAMS conditions. Given an input, the feedback is positive, if the end state after executing the input can shorten the distance so far. 
%
We estimate the distance optimistically so that the fuzzer that only climbs the hill can find stealthy vulnerabilities. 
%
We symbolize the input space of transactions and dynamically merge mempool states to reduce the search space.

We implement the fuzzing tool in Python and integrate it with popular Ethereum clients, including Geth, Nethermind, Besu, Erigon, Reth and OpenEthereum. 

\noindent{\bf 
Discovered exploits}: 
Running the fuzzer on Geth, Nethermind, Besu, Erigon, Reth and OpenEthereum leads to the discovery of XXX functional yet distinct exploits. Through manual analysis, we extract six attack patterns. 
First, our fuzzer can rediscover the known DETER attacks~\cite{DBLP:conf/ccs/LiWT21}, which evict the mempool by invalid transactions. 

Second, our fuzzer can discover a new pattern of stealthy attacks, transaction turning. The attacker sends two batches of transactions: The first batch consists of normal-looking valid transactions to evict the mempool, and the second batch of transactions to turn the first-batch transactions into invalid one, thus reducing the attack cost. In the discovered exploits, transactions can be turned by eviction or replacement. Unlike the existing DETER attacks, a turning attack consists of only valid transactions that are stealthier and can bypass checks to be propagated to all nodes.

Third, our fuzzer discovers a new class of low-cost locking attacks in which the attacker sends crafted transactions to occupy the empty slots in the victim mempool and lock it against subsequent normal transactions. Compared with eviction-based attacks, mempool locking achieves lower attack costs by uniquely exploiting order-sensitive admission policies (under which sending the same set of transactions but in different orders can lead to different admission results and mempool content).

\noindent{\bf
Attack evaluation}: While our exploits are discovered in a ``controlled'' setting (e.g., under synthetic transactions and running private blockchain nodes), we evaluate the effectiveness of these exploits in the wild.

By setting up attacker and measurement nodes in Goerli, we run experiments. The result shows that mounting a turning attack against a testnet achieves high success rates XXX at low attack cost XXX. Particularly, the crafted transaction in a turning attack, once sent in right timing, can be propagated to reach the entire network including the validator nodes.

%\ignore{
Against a mempool patched to mitigate turning attacks, one can send locking transactions with high success rates XXX. The cost of locking is XXX times lower than eviction attacks.

XXX

First, while deprecated, OpenEthereum's mempool is the most secure and can contain all DETER attacks under a low damage rate ($12.5\%$). By contrast, the new ADAMS attacks on OpenEthereum can achieve a much higher damage rate of $87.9$\textasciitilde{}$91.9\%$ and lower costs of $21,000$ Gas per block. 

We have disclosed the found bugs to the Ethereum developer community through bounty programs, and our bug reports have been confirmed.
%}

===

\noindent {\bf Mitigation design}:
Ideally, one may want to mitigate ADAMS attacks precisely (completely and soundly) to achieve both the security against ADAMS and the utility in preserving miner revenue. However, it is unattainable to execute this ideal mitigation scheme online, thanks to Ethereum's transaction model (refer to \S~\ref{sec:mitigate:intractible} for an example and the detailed discussion). Moreover, even for complete (and unsound) attack mitigation, the naive design that tracks the formation of all possible ADAMS attacks, while being a generic solution, can be too expensive to be executed online. 

We design a secure and lightweight mitigation scheme in two iterations: First, we start from a simple and domain-specific mitigation scheme F1 that enforces transaction priority at the mempool admission time. F1 prioritizes the admission of valid transactions over invalid ones and is designed to mitigate the ADAMS variants exploiting invalid transactions (i.e., circles and triangles in Figure~\ref{fig:seeds2}). Then, we propose lightweight attack detection called F2 to run on top of F1. F2 hardens the mempool against ADAMS variants that exploit low-cost valid transactions (i.e., the rectangle and diamond in Figure~\ref{fig:seeds2}). Specifically, F2 monitors the transaction trace, matches it to different attack patterns, estimates the success rate and cost of candidate patterns, and guides the mempool admission decision-making to avoid patterns of positive damage. 
Thanks to the duality among discovered attack patterns, the mempool may be trapped in a state with no possibility of preventing all ADAMS attacks. In this situation, we make our best efforts and suggest the admission decision with minimal damage.

We implement the attack detection/mitigation in a retrofittable subsystem over Geth with little instrumentation. The attack detection scheme is a pre-check on Geth's admission decision on any incoming transaction: If the decision is rejected, the scheme further recommends executing a safer admission decision.

\noindent {\bf Mitigation evaluation}: 
Through analysis and experiment, we evaluate the security of proposed online mitigation schemes. The result shows that a mempool hardened by F1 and F2 can mitigate the ADAMS patterns generated from our exploit-generation framework, pushing each potential attack's success rate to be $0\%$ or its attack cost to be as high as the baseline transaction spamming~\cite{DBLP:conf/fc/BaqerHMW16}. 

Our evaluation also verifies the duality among attacks by showing that partial mitigation (e.g., running F1 only) does not secure the mempool against all ADAMS attacks. For instance, on a Geth hardened with F1, the mempool locking attack using the low-cost valid transactions (i.e., rectangle in Figure~\ref{fig:seeds2}) can succeed with a $100\%$ rate at a cost lower than the baseline spamming by order of magnitude.

%The experience of hardening Geth with multiple design iterations reveal that securing a real-world mempool against all ADAMS attacks is a non-trivial task  

\noindent{\bf Contributions}: The paper makes contributions as follows:

\vspace{2pt}\noindent$\bullet$\textit{ 
New attacks}: Discovered new attack patterns in the previously unexplored design space to deny Ethereum's mempool service at a symmetric low cost. Built automatic exploit generation tools to adaptive generate and synthesize transaction traces against real-world Ethereum clients. Evaluated the effectiveness and low cost of the new attacks on the latest Ethereum clients patched secure against the known attacks. Also evaluated the effectiveness of the new attacks in denying mining services and propagating malicious transactions in the testnet.

\vspace{2pt}\noindent$\bullet$\textit{ 
Non-trivial defense}: Designed a suite of online migration schemes. Identified the duality among attack patterns and proposed a lightweight online detection scheme. Implemented the mitigation schemes on top of the Geth client. Evaluated the security by showing it can mitigate all discovered attacks.

XXX: In this work, we propose automatically discovering ADAMS vulnerabilities and exploits against actual mempool implementations in Ethereum clients. We first build an ``offline'' mempool testing tool that explores a blackbox mempool's input space, evades implementation-specific protections, and synthesizes exploits. We propose online schemes that mitigate the discovered ADAMS exploits and cause low performance interference. 

\ignore{
}



==> text/list_causes.tex <==

\newcommand{\tikzmarkvertical}[1]{\tikz[overlay,remember picture] \node (#1) {};}
\newcommand{\DrawBox}[1][]{%
        \tikz[overlay,remember picture]{      
        \draw[red,#1]
          ($(left1)+(-0.5em,1.6ex)$) rectangle
          ($(right1)+(0.5em,-0.6ex)$);
        \draw[red,#1]
          ($(left2)+(-0.5em,1.6ex)$) rectangle
          ($(right2)+(0.5em,-0.6ex)$);
        \draw[red,#1]
          ($(left16)+(-0.5em,1.6ex)$) rectangle
          ($(right16)+(0.5em,-5.95ex)$);
        \draw[red,#1]
          ($(left17)+(-0.5em,1.6ex)$) rectangle
          ($(right17)+(0.5em,-5.90ex)$);
        \draw[red,#1]
          ($(left3)+(-0.5em,1.6ex)$) rectangle
          ($(right3)+(0.5em,-0.6ex)$);
        \draw[red,#1]
          ($(left4)+(-0.5em,1.6ex)$) rectangle
          ($(right4)+(0.5em,-19.0ex)$);
        %\draw[red,#1]
        %  ($(left5)+(-0.5em,1.4ex)$) rectangle
        %  ($(right5)+(0.5em,-0.5ex)$);
        \draw[red,#1]
          ($(left6)+(-0.5em,1.6ex)$) rectangle
          ($(right6)+(0.5em,-3.2ex)$);
        %\draw[red,#1]
        %  ($(left7)+(-0.5em,1.4ex)$) rectangle
        %  ($(right7)+(0.5em,-0.5ex)$);
        \draw[red,#1]
          ($(left8)+(-0.5em,1.6ex)$) rectangle
          ($(right8)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left9)+(-0.5em,1.6ex)$) rectangle
          ($(right9)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left10)+(-0.5em,1.6ex)$) rectangle
          ($(right10)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left18)+(-0.5em,1.6ex)$) rectangle
          ($(right18)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left11)+(-0.5em,1.6ex)$) rectangle
          ($(right11)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left12)+(-0.5em,1.6ex)$) rectangle
          ($(right12)+(0.5em,-3.2ex)$);
        \draw[green,#1]
          ($(left14)+(-0.5em,1.6ex)$) rectangle
          ($(right14)+(0.5em,-0.6ex)$);
        \draw[green,#1]
          ($(left15)+(-0.38em,1.6ex)$) rectangle
          ($(right15)+(0.38em,-0.6ex)$);
        %\draw[red,#1]
        %  ($(left10)+(-0.5em,1.4ex)$) rectangle
        %  ($(right10)+(0.5em,-0.5ex)$);
        %\draw[red,#1]
        %  ($(left11)+(-0.5em,1.4ex)$) rectangle
        %  ($(right11)+(0.5em,-0.5ex)$);
        %\draw[red,#1]
        %  ($(left12)+(-0.5em,1.4ex)$) rectangle
        %  ($(right12)+(0.5em,-0.5ex)$);
        \draw[red,#1]
          ($(left13)+(-0.5em,1.6ex)$) rectangle
          ($(right13)+(0.5em,-0.6ex)$);

        }
        }


\renewcommand{\arraystretch}{1.2}
\begin{table*}[!htbp]
  \caption{Root causes of found exploits expressed by symbolized admission patterns (SAP).}
  \label{tab:causes}
  \centering{\footnotesize
  \begin{tabularx}{0.825\textwidth}{|l|X|*{10}{c}|}
  \hline
Name&Pattern & $XT_1$ & $XT_2$ & $XT_3$ &$XT_4$ & $XT_5$ & $XT_6$ & $XT_7$ & $MN_*$  & $XT_9$ & $XT_8$\\ \hline
   $SAP_1$& $[\mathcal{C}|\mathcal{P}] \rightarrow \mathcal{F}$ & \tikzmarkvertical{left1} \cmark \tikzmarkvertical{right1} & & \tikzmarkvertical{left16} \cmark \tikzmarkvertical{right16} && & & & \tikzmarkvertical{left9}\xmark\xmark \tikzmarkvertical{right9}& &\tikzmarkvertical{left4} \xmark\xmark \tikzmarkvertical{right4}\\ \hline 
$SAP_2$& $[\mathcal{C}|\mathcal{P}]\cdot{} [\mathcal{C}|\mathcal{P}] \rightarrow \mathcal{P}\cdot{}\mathcal{L}$ & &\tikzmarkvertical{left2} \cmark \tikzmarkvertical{right2}  & \cmark& && & &\tikzmarkvertical{left10}\xmark\xmark\tikzmarkvertical{right10} &&\xmark\xmark \\ \hline 
$CRP_1$ & (Conditional limit of txs per sender)  & &  & \cmark & &  &\tikzmarkvertical{left17} \cmark \tikzmarkvertical{right17}&&\tikzmarkvertical{left18}\xmark\xmark\tikzmarkvertical{right18} &&\xmark\xmark \\ \hline 
$SAP_4$& $\mathcal{P}\cdot\mathcal{C}\xrightarrow[]{\text{r}}\mathcal{P}\mathcal{L}$ & & &   & \tikzmarkvertical{left13} \cmark \tikzmarkvertical{right13}& & &&\tikzmarkvertical{left11}\xmark\xmark \tikzmarkvertical{right11}&&\xmark\xmark\\ \hline 
$SAP_5$& $\mathcal{P}\cdot{}\mathcal{C}\rightarrow\mathcal{F}\cdot{}[\mathcal{P}|\mathcal{C}]$ & &  & & & \tikzmarkvertical{left3} \cmark \tikzmarkvertical{right3}&\cmark& &\tikzmarkvertical{left12}\xmark\xmark \tikzmarkvertical{right12} & 
\tikzmarkvertical{left6} \xmark\xmark \tikzmarkvertical{right6}&\xmark\xmark\\ \hline 

$SAP_9$ & $\mathcal{P}_l \mathcal{C}_h \rightarrow{} \mathcal{P}_l \mathcal{P}_m$ & &  &  & &  && & \cmark & \xmark\xmark &\xmark\xmark\\ \hline 
$SAP_{11}$ & $C_l\rightarrow{}C_h$ &&&&&&&&\tikzmarkvertical{left15}\cmark\cmark\tikzmarkvertical{right15}&&\xmark\xmark\\ \hline 
$CRP_2$ & $\forall{SAP}, SAP\land{}\textsc{reversed}(SAP)$
 %(e.g.,  $\mathcal{P}_l\cdot\mathcal{C}_h \rightarrow{} \mathcal{P}_l \cdot \mathcal{P}_m \land{} \mathcal{P}_l \cdot \mathcal{P}_m \rightarrow{} \mathcal{P}_l \cdot\mathcal{C}_h$)
 & & && &  & &\tikzmarkvertical{left8} \cmark \tikzmarkvertical{right8} & \tikzmarkvertical{left14}\xmark\xmark \tikzmarkvertical{right14}  &&\xmark\xmark\\ \hline 
  \end{tabularx}
  }
\DrawBox[ultra thick]
\end{table*}



==> text/lst13_fuzz.tex <==
\begin{algorithm}[h]
\caption{Stateful Mempool Fuzzing}
\small \label{alg:fuzz2}
\hspace*{\algorithmicindent} \textbf{Input}: SeedDB $sdb$, Mempool $mp$
\begin{algorithmic}[1]
\While{!$sdb$.is\_empty() or timeout}
\State $st, ops$ = $sdb$.next(); \Comment{1. choose next seed}
\ForAll{$ops'$ = mutate($ops$, $st$)}
  \State $st'$ = execute($mp$, $ops'$);
\label{alg:fuzz2:exec}
  \If{is\_ADAMS\_exploit($st'$)} \Comment{3. test oracle}
    \State emit($ops'$, $st'$, "Found an exploit");
  \Else
    \If{!$sdb$.covers($st'$)} \Comment{2. state coverage}
        \State $sdb$.add($st'$, $ops'$);
    \EndIf
  \EndIf
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}



==> text/paper1_bw.tex <==
\vspace{-0.1in} \section{Introduction}
%In Ethereum, a mempool is a data structure buffering unconfirmed transactions from which block validators or builders select the transactions to be included in the next blocks. Mempool is essential in handling both public and private transactions in Ethereum 2.0. The denied service of a mempool can force the blockchain to produce low-Gas-utilization or even empty blocks and drop normal victim transactions sent from millions of web3 users, as observed recently~\cite{DBLP:conf/ccs/LiWT21}. The low-utilization blocks can undermine validators' incentives in mining and cause the shrinking of the blockchain network, re-introducing the 51\% attack vulnerabilities. 

In Ethereum, a mempool buffers unconfirmed transactions from web3 users before they are included in the next blocks. Mempool provides the essential functionality to bridge the gap between varying rates of submitted transactions and rates of produced blocks, regardless of public or private transactions it serves. As shown in recent studies~\cite{DBLP:conf/ccs/LiWT21}, denying a mempool service can force the blockchain to produce blocks of low or even zero (Gas) utilization, undermining validators' incentives and shrinking the blockchain networks in the long run, re-introducing the $51\%$ attacks. Besides, a denied mempool service can prevent normal transactions from block inclusion, cutting millions of web3 users off the blockchain and failing the decentralized applications relying on real-time blockchain access.

%ecent measurement studies~\cite{DBLP:journals/corr/abs-2203-15930,DBLP:journals/corr/abs-2208-02858} independently confirmed that only $2\%$ of transactions per block are private in Ethereum mainnets. 

\noindent{\bf Problem}: Spamming the mempool to deny its service has been studied for long~\cite{DBLP:conf/fc/BaqerHMW16,me:unconfirmed,DBLP:conf/icbc2/SaadNKKNM19,me:backlogged}. Early designs by sending spam transactions at high prices burden attackers with high costs and are of limited practicality. What poses a real threat is Asymmetric DeniAl of Mempool Service, coined by ADAMS, in which the mempool service is denied at an asymmetrically low cost. That is, the attack costs, in terms of the fees of adversarial transactions, are significantly lower than those of normal transactions victimized by the denied mempool. In the existing literature, DETER~\cite{DBLP:conf/ccs/LiWT21} is the first  ADAMS attack, and it works by sending invalid transactions to {\it directly evict} normal transactions in the mempool. MemPurge~\cite{cryptoeprint:2023/956} is a similar mempool attack that finds a way to send overdraft transactions into Geth's pending transaction pool and causes eviction there. 
These known attacks are easy to detect (i.e., following the same direct-eviction pattern). In fact, the DETER bugs reported in 2021 have been successfully fixed in all major Ethereum clients as of Fall 2023, including Geth, Nethermind, Erigon, and Besu. Given this state of affairs, we pose the following research question: 
Are there new ADAMS vulnerabilities in the latest Ethereum clients already patched against direct-eviction based attacks? 
%In other words, 
%Can patched Ethereum clients be asymmetrically DoS'ed by transaction patterns more sophisticated or stealthier than direct eviction in DETER? 

This work takes a systematic and semi-automated approach to discovering ADAMS vulnerabilities, unlike the existing DETER bugs that are manually found. 
Fuzzing mempool implementations is a promising approach but also poses unique challenges: 
Unlike the consensus implementation that reads only valid confirmed transactions, the mempool, which resides in the pre-consensus phase, needs to handle various unconfirmed transactions, imposing a much larger input space for the fuzzer. For instance, a mempool can receive \textit{invalid transactions under legitimate causes},\footnote{For instance, future transactions can be caused by out-of-order information propagation in Ethereum.} and factors such as fees or prices are key in determining transaction admission outcomes. Existing blockchain fuzzers including Fluffy~\cite{DBLP:conf/osdi/YangKC21}, Loki~\cite{DBLP:conf/ndss/MaCRZ00L023} and Tyr~\cite{me:tyr} all focus on fuzzing consensus implementation and don't explore the extra transaction space required by mempool fuzzing. As a result, directly re-purposing a consensus fuzzer to fuzz mempool would be unable to detect the DETER bugs as evaluated in Appendix \S~\ref{sec:motive}, let alone discover more sophisticated new ADAMS bugs.

%We observe that mempool fuzzing is not a code-coverage problem; for instance, the known ADAMS attack (i.e., DETER) that succeeds by repeating the same type of invalid transactions would repeatedly run the same code path of the mempool, without increasing the code coverage. 

\noindent{\bf 
Proposed methods}:
 To efficiently fuzz mempools, our key observation is that real-world mempool implementation admits transactions based on abstract ``symbols'', such as pending and future transactions, instead of concrete value. Thus, {\it sending multiple transactions under one symbol would trigger the same mempool behavior repeatedly}, and it suffices to explore just one transaction per symbol during fuzzing without losing the diversity of mempool behavior.

{  We propose symbolized-stateful mempool fuzzing or \textsc{mpfuzz}. 
To begin with, \textsc{mpfuzz} is set up and run in a three-step workflow: It is first manually set up against a size-reduced mempool under test, which induces a much smaller search space for fuzzing. Second, \textsc{mpfuzz} is iteratively run against the reduced mempool to discover short exploits. Third, the short exploits are manually extended to actual ones that are functional on real mempools and Ethereum clients. 
%
Internally, the design of \textsc{mpfuzz} is based on seven transaction symbols we design out of Ethereum semantics: future, parent, overdraft, latent overdraft, and replacement transactions. Under these symbols, in each iteration of fuzzing, \textsc{mpfuzz} explores one concrete transaction per symbol, sends the generated transaction sequence to the target mempool, observes the mempool end state, and extracts the feedback of symbolized state coverage and state promisingness in reaching bug oracles to guide the next round of fuzzing. In particular, \textsc{mpfuzz} employs a novel technique to evaluate state promisingness, that is, by {\it optimistically} estimating the costs of unconfirmed transactions whose validity is subject to change in the future. }

%We propose symbolized-stateful mempool fuzzing or \textsc{mpfuzz}. We first manually design seven symbols from Ethereum semantics to cover future, parent, child, overdraft, latent overdraft, and replacement transactions. Then, during fuzzing, \textsc{mpfuzz} generates a new transaction by symbol, sends the input to execute on a target mempool implementation, observes the end state of the mempool, and uses the symbolized state coverage as feedback to guide the next round of mutation. By this means, \textsc{mpfuzz} searches the space of symbolized mempool states for the one matching the bug oracles induced by ADAMS. To further speed up the search in a limited time, we prioritize ``promising'' states by {\it optimistically} estimating the costs of unconfirmed transactions whose validity is subject to change in the future.

%We propose \textsc{mpfuzz}, a symbolic and optimistic approach for stateful mempool fuzzing. \textsc{mpfuzz} uses as feedback the state coverage and how promising the state is in reaching a target state satisfying the test oracle. We {\it optimistically} estimate the promising-ness of a mempool state so that \textsc{mpfuzz} that climbs the hill can still find ``stealthy'' ADAMS attacks. 

\noindent{\bf 
Found attacks}:
{  
We run \textsc{mpfuzz} on six leading execution-layer Ethereum clients deployed on the mainnet's public-transaction path (Geth~\cite{me:geth}, Nethermind~\cite{me:nethermind}, Erigon~\cite{me:erigon}, Besu~\cite{me:besu}, Reth~\cite{me:reth}, and OpenEthereum~\cite{me:parity}), three PBS builders (proposer-builder separation) on the mainnet's private-transaction and bundle path (Flashbot $v1.11.5$~\cite{me:flashbotbuilder}, EigenPhi~\cite{me:eigenphibuilder} and bloXroute~\cite{me:bloXroutebuilder}), and three Ethereum-like clients (BSC $v1.3.8$~\cite{me:bscclient} deployed on Binance Smart Chain, go-opera $v1.1.3$~\cite{me:goopera} on Fantom, and core-geth $v1.12.19$~\cite{me:coregeth} on Ethereum Classic). 
}
Compared to the baseline fuzzers, \textsc{mpfuzz} can find exploits faster by more than two orders of magnitude. On Ethereum clients of historical versions, \textsc{mpfuzz} can rediscover known DETER bugs. On the latest Ethereum clients where DETER bugs are fixed, \textsc{mpfuzz} can find new ADAMS attacks, described next.

We summarize the newly discovered ADAMS exploits into several patterns: 1) Indirect eviction by valid-turned-invalid transactions. Unlike the direct-eviction pattern used in DETER, the indirect-eviction attack works more stealthily in two steps: The attacker first sends normal-looking transactions to evict victim transactions from the mempool and then sends another set of transactions to {\it turn} the admitted normal-looking transactions into invalid ones, bringing down the cost. 2) Locking mempool, which is to occupy the mempool to decline subsequent victim transactions. Mempool locking does not need to evict existing transactions from the mempool as the eviction-based DETER attacks do.
3) Adaptive attack strategies where the attack composes adversarial transactions in an adaptive way to the specific policies and implementations of the mempool under test. Example strategies include composing transactions of multiple patterns in one attack, re-sending evicted transactions to evict ``reversible'' mempools, locking mempool patched against turning, etc. 
%
 { We propose rule-based mitigation schemes against all newly discovered vulnerabilities.}

All newly found ADAMS bugs are reported to the developer communities, including Ethereum Foundation, BSC, Fantom, PBS builders, etc. with $15$ bugs confirmed and $4$ fixed in recent client releases~\cite{me:gethfix11}. 
Bug reporting is documented on the webpage~\cite{me:mpfuzz:report}, which also includes demos of \textsc{mpfuzz} on the tested Ethereum clients. \textsc{mpfuzz} will be open-sourced to facilitate vulnerability discovery in more and future clients.

\noindent{\bf Contributions}: The paper makes contributions as follows:

\vspace{2pt}\noindent$\bullet$\textit{ 
New fuzzing problem}: This paper is the first to formulate the mempool-fuzzing problem to automatically find asymmetric DoS vulnerabilities as bug oracles. Fuzzing mempools poses new unique challenges that existing blockchain fuzzers don't address and entails a larger search space including invalid transactions and varying prices. 



\vspace{2pt}\noindent$\bullet$\textit{ 
New fuzzing method}: The paper presents the design and implementation of \textsc{mpfuzz}, 
{ 
a symbolized-stateful mempool fuzzer. Given a mempool implementation, \textsc{mpfuzz} defines the search space by the mempool states covered under symbolized transaction sequences and efficiently searches this space using the feedback of symbolized state coverage and the promising-ness of an intermediate state in triggering bug oracles. } 
With a Python prototype and runs on real Ethereum clients, \textsc{mpfuzz} achieves a $>100\times$ speedup in finding known DETER exploits compared to baselines.

\vspace{2pt}\noindent$\bullet$\textit{ 
New discovery of mempool vulnerabilities}: \textsc{mpfuzz} discovers new asymmetric-DoS vulnerabilities in six major Ethereum clients in the mainnet. By evaluation under real transaction workloads, all found attacks achieve $84.6-99.6\%$ success rates and low costs such as adversarial transaction fees $100\times$ lower than the victim transaction fees.

\vspace{-0.1in} \section{Related Works}
\label{sec:rw}

\noindent{\bf 
Consensus fuzzers}:
Fluffy~\cite{DBLP:conf/osdi/YangKC21} is a code-coverage based differential fuzzer to find consensus bugs in Ethereum Virtual Machines (EVM). 
Specifically, given an EVM input, that is, a transaction sequence, Fluffy sends it to multiple nodes running different Ethereum clients (e.g., Geth and OpenEthereum) for execution. 
1) The test oracle in Fluffy is whether the EVM end states across these nodes are different, implying consensus failure.
%The states in Fluffy includes account Ether balance, contract account status, and other EVM states.
%This allows Fluffy to find bugs due to flawed interactions between Ether balance and smart contracts.
2) Fluffy mutates ordered transaction sequences at two levels: it reorders/adds/deletes transactions in the sequence, and for each new transaction to generate, it randomly selects values in Gas limits and Ether amounts. For the data field, it employs semantic-aware strategies to add/delete/mutate bytecode instructions of pre-fixed smart contract templates. 
3) Fluffy uses code coverage as feedback to guide the mutation.

Loki~\cite{DBLP:conf/ndss/MaCRZ00L023} is a stateful fuzzer to find consensus bugs causing crashes in blockchain network stacks.
%
Specifically, Loki runs as a fuzzer node interacting with a tested blockchain node through sending and receiving network messages.
1) The test oracle in Loki is whether the tested blockchain node crashes. 
2) The fuzzer node uses a learned model of blockchain network protocol to generate the next message of complying format, in which the content is mutated by randomly choosing integers and bit-flipping strings. In other words, the mutation in Loki is unaware of application level semantics. For instance, if the message is about propagating an Ethereum transaction, the transaction's nonce, Ether amount, and Gas price are all randomly chosen; the sender, receiver, and data are bit flipped.
3) Loki records messages sent and received from the test node. It uses them as the state. New states receive positive feedback.

Tyr~\cite{me:tyr} is a property-based stateful fuzzer that finds consensus bugs causing the violation of safety, liveness, integrity, and other properties in blockchain network stacks.
%
Specifically, in Tyr, a fuzzer node is connected to and executes a consensus protocol with multiple neighbor blockchain nodes. 
1) The test oracle Tyr uses is the violation of consensus properties, including safety (e.g., invalid transactions cannot be confirmed), liveness (e.g., all valid transactions will be confirmed), integrity, etc. The checking is realized by matching an observed end state with a ``correct'' state defined and run by the Tyr fuzzer.
2) Tyr mutates transactions on generic attributes like randomly selecting senders and varying the amount of cryptocurrencies transferred (specifically, with two values, the full sender balance, and balance plus one). When applied to Ethereum, Tyr does not mutate Ethereum-specific attributes, including nonce or Gas price. It generates one type of invalid transaction, that is, the double-spending one, which in account-based blockchains like Ethereum are replacement transactions of the same nonce. 
3) Tyr uses state divergence as the feedback, that is, the difference of end states on neighbor nodes receiving consensus messages in the same iteration. In Tyr, the states on a node include both the messages the node sent and received, as well as blocks, confirmed transactions, and other state information.

These existing blockchain fuzzers~\cite{me:tyr,DBLP:conf/ndss/MaCRZ00L023,DBLP:conf/osdi/YangKC21} cannot detect mempool DoS bugs and are different from this work. Briefly, mempool DoS does not trigger system crashes and can not be detected by Loki. Mempool content difference across nodes does not mean insecurity, and the mempool DoS bugs can not be detected by Fluffy (which detects consensus state difference). 
While Tyr aims to detect liveness and safety violations, their model of invalid transactions is rudimentary. Specifically, they only model double-spending transactions and cannot detect DETER bugs~\cite{DBLP:conf/ccs/LiWT21} that rely on more advanced invalid transactions, like future transactions and latent overdrafts.

\noindent{\bf
Blockchain DoS}: Blockchain DoS security has been examined at different system layers, including P2P networks~\cite{DBLP:conf/uss/HeilmanKZG15,DBLP:journals/iacr/MarcusHG18,DBLP:conf/sp/ApostolakiZV17,tran2020stealthier}, mining-based consensus~\cite{mirkin2019bdos,me:finney}, and application-level smart contracts~\cite{DBLP:conf/ndss/0002L20,me:eip150,me:dosblockgas} and DApp (decentralized application) services~\cite{DBLP:conf/ndss/LiCLT0L21}. These DoSes are not related to mempools and are orthogonal to this work.

For mempool DoS, a basic attack is by sending spam transactions with high fees to evict victim transactions of normal fees~\cite{DBLP:conf/fc/BaqerHMW16,me:unconfirmed,DBLP:conf/icbc2/SaadNKKNM19,me:backlogged}, which incur high costs to attackers. DETER~\cite{DBLP:conf/ccs/LiWT21} is the first asymmetric DoS on Ethereum mempool where the adversary sends invalid transactions of high fees (e.g., future transactions or latent overdrafts) to evict victim transactions of normal fees. Concurrent to this work is MemPurge~\cite{cryptoeprint:2023/956} posted online in June 2023; in it, the attacker reconnects her adversarial future transactions and makes them latent-overdraft transactions. 
The DETER bugs have been fixed on the latest Ethereum clients such as Geth $v1.11.4$, as we tested them in July 2023. Both DETER and MemPurge are manually discovered. 
%
{More related work is deferred to Appendix~\ref{appdx:more-related-work}.}

{
\vspace{-0.1in} \section{Background}


\noindent{\bf Ethereum mempools}:
In Ethereum, users send their transactions to the blockchain network, which are propagated to reach validator nodes. On every blockchain node, unconfirmed transactions are buffered in the mempool before they are included in the next block or evicted by another transaction.
In Ethereum 2.0, transactions are propagated in two fashions: public transactions are broadcast among all nodes, and private transactions are forwarded to selected nodes, more specifically, selected builders and proposers (as in PBS or proposer-builder separation).
The mempool is present on both paths, and it is inside Ethereum clients such as Geth~\cite{me:geth} and Nethermind~\cite{me:nethermind} (handling public transactions), and Flashbot~\cite{me:flashbotbuilder} (private transactions).
On these clients, a mempool also serves many other downstream modules, including MEV searchers or bots (in PBS), Gas stations, RPC queries, etc.

Mempools on different nodes are operated independently and don't need to synchronize as the consensus layer does. For instance, future transactions are not propagated, and the set of future transactions in the mempool on one node is different from another node.

The core mempool design is transaction admission: Given an initial state, whether and how the mempool admits an arriving transaction. In practice, example policies include those favoring admitting transactions of higher prices (and thus evicting or declining the ones of lower prices), transactions arriving earlier, certain transaction types (e.g., parent over child transactions), and valid transactions (over future transactions). See different types of Ethereum transactions in \S~\ref{sec:notations}.
}

{
%
\noindent{\bf 
Transactions and fees}: Given an Ethereum transaction $tx$, its fee is the product of $GasUsed$ and $GasPrice$, that is, $tx.fee=GasUsed*GasPrice$. 
$tx.GasUsed$ is the sum of a fixed $21000$ Gas (for computation done for basic transaction validation) and a variable amount proportional to the computations caused by smart-contract execution in $tx$. $GasUsed$ is determined only after the execution of $tx$. 
Typically, a transaction is executed when selected to be included in the next block, and the fees of the transaction are charged when the next block is finalized with sufficient confirmations.

In Ethereum, the sender of $tx$ may also set $tx.Gas$, which is the upper bound of $GasUsed$.
After EIP-1559, $GasPrice=BaseFee+PriorityFee$, where the $BaseFee$ is decided by the blockchain and its associated fees are burnt upon transaction inclusion. The validator collects the rest of the fees, namely, $GasUsed*(PriorityFee)$ or $tip$.
}

\vspace{-0.1in} \section{Threat Model and Bug Oracle}
\label{sec:threatmodel}

{
 
In the threat model, an attacker controls one or few nodes to join an Ethereum network, discovers and neighbors critical nodes (e.g., top validators, backends of an RPC Service, MEV searcher) if necessary, and sends crafted adversarial transactions to their neighbors. The attacker in this work has the same networking capacity as in DETER~\cite{DBLP:conf/ccs/LiWT21}.

The attacker's goal is to disable the mempools on the critical nodes or all nodes in an Etheurem network and cause damage such as deployed or dropped transactions in block inclusion, produced blocks of low or zero (Gas) utilization, and disabled other downstream services like MEV searchers. In practice, this damage is beneficial to competing block validators, MEV searchers, and RPC services. Besides, the attacker aims to cause this damage at asymmetrically low costs, as will be described. 
}

\ignore{
In the threat model, an attacker controls one or a few nodes joining a target Ethereum network. The attacker's goal is to disable some critical functions in the entire network, including the block production (or mining) and relay of submitted transactions through RPC services. Specifically, in either case of disabling network-wide block production or RPC Service, a successful ADAMS attack can result in the blockchain appended with empty blocks. 

The attacker has the capability of joining nodes in the target Ethereum network,  propagating transactions in the network, and passively observing the traffic of messages that are received by or sent by the attack nodes. Using these capabilities, the attacker may be able to discover critical service nodes running behind the popular RPC infrastructures and top mining pools, which is feasible in the pre-merge Ethereum network~\cite{DBLP:conf/ccs/LiWT21}. 

We describe the attack design goals: 1) Against a given victim node, the attacker aims to find crafted transactions to be sent to the victim and to deny its mempool service to the local miner (or block producer). So, the local miner reads zero unconfirmed transactions and proposes empty blocks. 2) Optionally, the attacker aims at finding the craft transactions that will be propagated. That is, the victim node receiving the crafted transactions would propagate them to its neighbor nodes, and so do the neighbors until the crafted transactions are propagated to the entire network.

While causing the DoS damage to the Ethereum network, an ADAMS attacker aims at achieving asymmetrically low cost, that is, the fees of crafted transactions sent in an attack must be significantly lower than those of victim transactions, either evicted or declined upon admission. 
}

\vspace{-0.1in} \subsection{Notations}
\label{sec:notations}

\noindent{\bf 
Transactions}:
In Ethereum, we consider two types of accounts: a benign account of index $i$ denoted by $B_i$, and an adversarial account of index $i$ denoted by $A_i$. A (concrete) Ethereum transaction $tx$ is denoted by $tx{\begin{reduce}\begin{bsmallmatrix}{s} & {v}\\ {n} & {f}\end{bsmallmatrix}\end{reduce}}$, where the sender is $s$, the nonce is $n$, the Gas price is $f$, and the transferred value in Ether is $v$.
This work does not consider the ``data'' field in Ethereum transactions or smart contracts because smart contracts do not affect the validity of the Ethereum transaction. The notations are summarized in Table~\ref{tab:notations}.

\begin{table}[!htbp] %force in current page, disable float.
\caption{Notations}
\label{tab:notations}\centering{\small
\begin{tabularx}{0.475\textwidth}{ |l|X|l|X| }
  \hline
Symbol & Meaning & Symbol & Meaning  \\ \hline
$m$ & Mempool length 
&
$ops$ & Tx sequence
 \\ \hline
$st$ & State of residential txs in mempool
&
$dc$ & History of declined txs from mempool
 \\ \hline
$A$ & Adversarial tx sender
&
$B$ & Benign tx sender
 \\ \hline
&\multicolumn{3}{p{2in}|}{}\\[-0.8em]
  $tx\begin{bsmallmatrix}{s} & {v}\\ {n} & {f}\end{bsmallmatrix}$
  & 
  \multicolumn{3}{p{2.5in}|}{
A transaction from sender $s$, of nonce $n$, transferring Ether value $v$, and with Gas Price $f$
}
 \\ \hline
\end{tabularx}
}
\end{table}

We use each of the following symbols to represent a disjoint group of transactions. Informally, $\mathcal{N}$ is a transaction sent from a benign account, $\mathcal{F}$ a future transaction, $\mathcal{P}$ a parent transaction, $\mathcal{C}$ a child transaction, $\mathcal{O}$ an overdraft transaction, $\mathcal{L}$ a latent overdraft transaction, and $\mathcal{R}$ a replacement transaction. These symbols are formally specified in \S~\ref{sec:symbolize}.

Particularly, we use the notion of latent overdraft from the existing work~\cite{DBLP:conf/ccs/LiWT21}, which indicates a child transaction that by itself does not overdraft but does overdraft when taking into account its parent transactions. Suppose Alice has a balance of $5$ Ether and sends $tx_1$ of nonce $1$ spending $2$ Ether and $tx_2$ of nonce $2$ spending $4$ Ether. $tx_2$ is a latent overdraft.

\noindent{\bf 
States and transitions}: We recognize two mempool-related states in Ethereum, the collection of transactions stored in mempool $st$, and the collection of declined transactions $dc$. 

Suppose a mempool of state $\langle{}st_i, dc_i\rangle{}$ receives an arriving transaction $tx_i$ and transitions to state $\langle{}st_{i+1}, dc_{i+1}\rangle{}$. 

An arriving transaction can be admitted with eviction, admitted without eviction, or declined by a mempool. The three operations are defined as follows. 1) An arriving transaction $tx_i$ is admitted with evicting a transaction $tx_i'$ from the mempool, if 
$st_{i+1}=st_{i}\setminus{}tx_i'\cup{}tx_i,dc_{i+1}=dc_i$.
2) $tx_i$ is admitted without evicting any transaction in the mempool, if 
$st_{i+1}=st_{i}\cup{}tx_i,dc_{i+1}=dc_i$.
3) $tx_i$ is declined and does not enter the mempool, if 
$st_{i+1}=st_{i},dc_{i+1}=dc_i\cup{}tx_i$.

\begin{figure}[!bthp]
\centering
%\includegraphics[width=0.49\textwidth]{figures/tx-space.eps}
\includegraphics[width=0.41\textwidth]{figures/mpfuzz-overview.eps}
%\includegraphics[width=0.32\textwidth]{figures/mpfuzz-overview2.eps}
%\includegraphics[width=0.475\textwidth]{figures/mpfuzz-overview3.eps}
\caption{Overview of exploit discovery and evaluation workflow: 0) \textsc{mpfuzz} setup, 1) mempool reduction, 2) fuzzing on reduced mempool under test (MUT) to discover short exploits, and 3) exploit extension. The extended exploits are 4) evaluated on the actual mempool of the original size. Green means automated tasks, and gray requires manual effort.}
\label{fig:overview}
\end{figure}

 
{ 
\vspace{-0.1in} \subsection{Exploit Discovery Workflow}

To set up the stage, we present the workflow overview in this work. The workflow is depicted in Figure~\ref{fig:overview}. To discover vulnerabilities and exploits in an actual mempool, one has to 0) set up \textsc{mpfuzz} by various parameters (as will be introduced), 1) reduce the mempool from its original configuration to a much smaller version, named mempool under test (MUT). 2) \textsc{mpfuzz} is run on the reduced MUT deployed locally (with settings described in \S~\ref{sec:mut:setting}). Fuzzing leads to the discovery of short exploits. 3) Short exploits are extended to the longer ones, that is, actual exploits. 4) The success of the actual exploit is evaluated on the actual mempools deployed in close-to-operational settings, such as using popular Ethereum testnets like Goerli (see \S~\ref{sec:evaluate:testnet}) or a network we set up locally running unmodified Ethereum clients (see \S~\ref{sec:evaluate:locking} and Appendices \S~\ref{appdx:sec:eval:locking2} and \S~\ref{appdx:sec:additional-attack-evaluation}).
%
Fuzzing a reduced mempool (MUT) instead of an original one is necessary to ensure the efficient execution of the \textsc{mpfuzz}, which entails many iterations of re-initiating and populating the mempool. We discuss and evaluate the possible false positives that could be introduced by fuzzing smaller MUT in \S~\ref{sec:falsepositives}.

In this workflow, fully automated is Step 2), that is, the discovery of short exploits on a given MUT (colored green in Figure~\ref{fig:overview}). Other steps colored in gray require manual efforts and are described below:
%
In {\bf Step 0)}, \textsc{mpfuzz} setup entails setting parameters in bug oracles (e.g., $\epsilon$ and $\lambda$) and fixed symbols in guiding fuzzing. The setup is usually one-time.
%
In {\bf Step 1)}, mempool reduction entails reconfiguring the mempool to a much smaller capacity (e.g., MUT length $m=6$ or $m=16$, compared to the original size like $m'=6144$ as in Geth). In addition, policy-specific parameters in the actual mempool are tuned down proportionally. For instance, the Geth mempool buffers up to $py_1'=1024$ future transactions, and when buffering more than $py'_3=5120$ pending transactions, the mempool triggers a protective policy to limit the number of transactions sent from the same sender by $py_2'=16$ . In a reduced MUT of $m=6$, these parameters are reduced while retaining the same proportion, such as $py_1=1, py_3=5, py_2=2$. The mempool reduction requires expert understanding and manual efforts, and it is by nature the best effort.
%
In {\bf Step 3)}, it first de-duplicates the raw short exploits found by \textsc{mpfuzz}. Then, for each distinct short exploit, it extends it by repeating the transaction-admission events to fit into the actual mempool, during which one may practice strategies like increasing nonce, switching sender accounts, and measuring normal transactions in the actual mempool. In exploit extension, one could also consider the factors not modeled in MUT or \textsc{mpfuzz} such as $BaseFee$, as seen in the case in \S~\ref{sec:eval:locking:xt8a}.
}

{
\vspace{-0.1in} \subsection{Bug Oracle: Definitions \& Rationale}
\label{sec:oracle}

\begin{definition}[Tx admission timeline]
\label{def:timeline}
In a transaction admission timeline, a mempool under test is initialized at state $\langle{}st_0, dc_0=\emptyset\rangle{}$, receives a sequence of arriving transactions $ops$, and ends up with state $\langle{}st_n, dc_n\rangle{}$. Then, a validator continually builds blocks by selecting and clearing transactions in the mempool until the mempool is empty. This transaction timeline is denoted by $\langle{}st_0, dc_0=\emptyset\rangle{}, ops\Rightarrow{}\langle{}st_n, dc_n\rangle{}$. 
\end{definition}

The transaction admission timeline is simplified from the timeline that an operational mempool experiences where transaction arrival and block building can be interleaved. The simplification is intended to trade off the accuracy of fuzzing results for fuzzing efficiency as discussed in  \S~\ref{sec:falsepositives}.

We use two mempool-attack templates to define two bug oracles: an eviction-based DoS where adversarial transactions evict existing victim transactions in the mempool, and a locking-based DoS where existing adversarial transactions in the mempool decline arriving victim transactions.

\begin{definition}[Eviction bug oracle]
\label{def:oracle:evict}
A transaction admission timeline, $\langle{}st_0, dc_0=\emptyset\rangle{}, ops \Rightarrow{}\langle{}st_n, dc_n\rangle{}$, is a successful \textsc{ADAMS} eviction attack, if.f. 1) the admission timeline causes full damage, that is, initial state $st_0$ contains only benign transactions, 
$ops$ are adversarial transactions, and the result end state $st_n$ contains only adversarial transactions (in Equation~\ref{eqn:adams:evict:1}), and 2) the attack cost is asymmetrically low, that is, the total adversarial transaction fees in the end state $st_n$ to be charged are smaller, by a multiplicative factor $\epsilon$, than the attack damage measured by the fees of evicted transactions in the initial state $st_0$ (in Equations~\ref{eqn:adams:evict:2} and~\ref{eqn:adams:evict:3}). Formally, 

\begin{eqnarray}
\label{eqn:adams:evict:1}
st_0\cap{}st_n &=& \emptyset 
\\
\label{eqn:adams:evict:2}
asym_E(st_0, ops) &\stackrel[]{def}{=}& \frac{\sum_{tx\in{}st_n}tx.fee}{\sum_{tx\in{}st_0}tx.fee} 
\\
\label{eqn:adams:evict:3}
asym_E(st_0, ops) &<& \epsilon
\end{eqnarray}
\end{definition}

\begin{definition}[Locking bug oracle]
\label{def:oracle:lock}
A transaction admission timeline, $\langle{}st_0=\emptyset, dc_0=\emptyset\rangle{}, ops \Rightarrow{}\langle{}st_n, dc_n\rangle{}$, is a successful \textsc{ADAMS} locking attack, if.f. 1) the admission timeline causes full damage, that is, the mempool is first occupied by adversarial transactions (i.e., $st_n$ contains only adversarial transactions) and then declines the arriving normal transactions (i.e., $dc_n$ contains only normal transactions); the normal transactions and adversarial transactions are sent by different accounts (i.e., Equation~\ref{eqn:adams:decline:1}), and 2) the attack cost is asymmetrically low, that is, the average adversarial transaction fees in the mempool are smaller, by a multiplicative factor $\lambda$, than the attack damage measured by the average fees of victim transactions declined (i.e., Equations~\ref{eqn:adams:decline:2} and~\ref{eqn:adams:decline:3}).
Formally, 

\begin{eqnarray}
%\cup_{txd\in{}dc_n}{txd.sender} \; \cap && \\ 
%\cup_{txd\in{}dc_n}{txd.sender}  &\cap &
\cup_{tx\in{}dc_n}{tx.sender}  &\cap &
\cup_{tx\in{}st_n}{tx.sender} = \emptyset
\label{eqn:adams:decline:1}  
\\ 
asym_D(ops) &\stackrel[]{def}{=}& 
\frac{\sum_{tx\in{}st_n} tx.fee / \|st_n\|}{\sum_{tx\in{}dc_n}tx.fee / \|dc_n\|}
\label{eqn:adams:decline:2}
\\
asym_D(ops) &<& \lambda 
\label{eqn:adams:decline:3}
\end{eqnarray}
\end{definition}


\noindent{\bf Design rationale}: Both definitions use the normal transaction fees to measure the attack damage because these fees are not collected by the validator in the timeline under attack and are collectible without attack. Specifically, the damage in Definition~\ref{def:oracle:evict} is measured by the fees of normal transactions in $st_0$ which are evicted in end state $st_n$ and which would not have been evicted had there been no adversarial transactions in $ops$. The damage in Definition~\ref{def:oracle:lock} is measured by the fees of normal transactions in $ops$ which are declined from end state $st_n$ and which would not have been declined had there been no adversarial transactions in $ops$.

Both definitions are strict and require causing full damage, such as evicting or declining {\it all} normal transactions. Strict definitions are necessary to ensure that what is found as exploits on the small MUT is true positive and works on the actual mempool. Appendix \S~\ref{sec:oracle:relaxed} discusses relaxing the design of bug oracles.

The targeted attacks by this work are denial of mempool service in feeding downstream validators with valid transactions sent from benign users. They are different from other forms of DoS in blockchains, including resource exhaustion via executing malicious smart contracts~\cite{cryptoeprint:2023/956,DBLP:conf/ndss/LiCLT0L21}.

Particularly, in the threat model of mempool DoS, we assume the validators are benign and functional in building blocks. Because in all Ethereum clients we know, transactions are admitted into mempool without execution (i.e., executing the smart contracts they invoke), $GasUsed$ is not a factor in transaction admission.\footnote{The further design rationale for admitting transactions without execution is that an Ethereum transaction $tx$'s $GasUsed$ is non-deterministic unless the ordering of $tx$ w.r.t. other transactions in the block is fixed and $tx$ is executed.} Thus, our bug oracle does not vary $GasUsed$. Instead, all the transactions are fixed at $21000$ Gas (i.e., as if they don't invoke smart contracts).\footnote{We may use price and fees interchangeably.} This design significantly reduces the search space without loss in covering different mempool behaviors.
%The transactions of varying fees are those of varying prices. We leave it to future work to model contract-executing transactions or transactions of varying $GasUsed$.
Besides, our bug oracle does not model the effect of EIP1559 or $BaseFee$. Without modeling $BaseFee$, our bug oracle can still capture the alternative transaction fee (the product of Gas price and $21000$ Gas), which is still proportional to actual $tip$ or damage on validator revenue. }


\vspace{-0.1in} \section{Stateful Mempool Fuzzing by \textsc{mpfuzz}}
\label{sec:symbolize}

\vspace{-0.1in} \subsection{Transaction Symbolization}

The key challenge in designing \textsc{mpfuzz} is the large input space of transaction sequences. Recall that an Ethereum transaction consists of multiple attributes (sender, nonce, Gas price, value, etc.), each defined in a large domain (e.g., 64-bit string). Exploring the raw transaction space is hard; the comprehensive search is inefficient, and randomly trying transactions as done in the state-of-the-art blockchain fuzzers (in \S~\ref{sec:rw}) is ineffective.

\noindent{\bf
Intuition}: We propose symbolizing transactions for efficient and effective mempool stateful fuzzing. Our key idea is to map each group of concrete transactions, triggering an equivalent mempool behavior into a distinct symbol so that searching for one transaction is sufficient to cover all other transactions under the same symbol. Transaction symbolization is expected to reduce the search space from possible concrete transactions to the symbol space.

{  
In this work, we manually design seven symbols to represent Ethereum transactions based on the Ethereum ``semantics'', that is, how different transactions are admitted by the mempool. Our manually crafted transaction symbols are evaluated to be consistent with Ethereum semantics, as shown in Appendix~\ref{appdx:transaction-code-coverage}. 
}

%\noindent{\bf Mempool model}: To motivate the design of our transaction symbols, we first describe an abstracted and common mempool model. The mempool runs the following admission policies: 1) {\bf Policy $py_0$}: Given an incoming transaction $tx_1$, upon a full mempool, it finds the transaction of the lowest fee, say $tx_2$, and decides to admit $tx_1$ by evicting $tx_2$ if $tx_1$'s fee is higher than $tx_2$'s fee. 2) {\bf Policy $py_2$}: The mempool limits the number of future transactions. By default, a Geth mempool of the capacity of $n=5120+1024$ transactions can store up to $py_2=1024$ future transactions. 
%To enforce this property, Geth implements several rules, such as declining a future transaction upon arrival if the mempool already has 1024 future transactions and keeping evicting extra future transactions until below 1024 future transactions in the mempool upon each transaction admission. 3) {\bf Policy $py_3$}: The mempool limits the number of pending transactions sent from the same sender. By default, this policy is conditional and is triggered when more than $py_3'=5120$ pending transactions exist in the mempool. It limits $py_3=16$ transactions per sender account. 

\begin{table}[!htbp] %force in current page, disable float.
 \caption{Symbols, transactions, and associated costs. Tx refers to the instantiated transaction under a given symbol.}
\label{tab:symbols:2}\centering{\small
\begin{tabularx}{0.49\textwidth}{ l|l|X|l|l }
Symbol        & Description & Tx  & $cost()$ & $opcost()$ \\ \hline 
&&&&\\[-0.8em]
$\mathcal{N}$ & Benign & $tx{\begin{reduce}\begin{bsmallmatrix}{B*} & {1}\\ {*} & {3}\end{bsmallmatrix}\end{reduce}}$ & $3$ & $3$ \\ [3pt]\hline 
&&&&\\[-0.8em]
$\mathcal{F}$ & Future & $tx{\begin{reduce}\begin{bsmallmatrix}{A*} & {1}\\ {m+1} & {m+1}\end{bsmallmatrix}\end{reduce}}$ & $0$ & $0$ \\ [3pt]\hline 
&&&&\\[-0.8em]
$\mathcal{P}$ & Parent & $tx{\begin{reduce}\begin{bsmallmatrix}{A>r} & {1}\\ {1} & {[4,m]}\end{bsmallmatrix}\end{reduce}}$& $[4, m]$ & $[4,m]$ \\ [4pt]\hline 
&&&&\\[-0.8em]
$\mathcal{C}$ & Child & $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$ & $m+1$ & {\color{red} $1$} \\ [4pt]\hline 
&&&&\\[-0.8em]
$\mathcal{O}$ & Overdraft & $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m+1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$ & $0$ & $0$ \\ [4pt]\hline 
&&&&\\[-0.8em]
$\mathcal{L}$ & Latent overdraft & $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m-1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$ & $0$ & $0$ \\ [4pt] \hline 
&&&&\\[-0.8em]
$\mathcal{R}$ & Replacement & $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m-1}\\ {1} & {m+1}\end{bsmallmatrix}\end{reduce}}$ & $0$ & $0$  \\ [4pt]\hline
\end{tabularx}}
\end{table}

\noindent{\bf 
Specification}: Suppose the current state contains adversarial transactions sent from $r$ accounts $A_1,\dots, A_r$. 
These accounts have an initial balance of $m$ Ether, where $m$ equals the mempool capacity (say $m=1000$).
{ 
The rationale is that these accounts can send at most $m$ adversarial transactions, each minimally spending one Ether, to just occupy a mempool of $m$ slots. A larger value of attacker balance is possible but increases the search space.
}

Symbol $\mathcal{N}$ defines a transaction subspace covering any normal transactions sent from any benign account and of any nonce, namely $tx\begin{bsmallmatrix}{B*} & {*}\\ {*} & {*}\end{bsmallmatrix}$
. In \textsc{mpfuzz}, Symbol $\mathcal{N}$ is instantiated to concrete transactions of fixed Gas price $3$ wei and of value $1$ Ether. That is, symbol $\mathcal{N}$ is instantiated to transaction $tx\begin{bsmallmatrix}{B*} & {1}\\ {*} & {3}\end{bsmallmatrix}$
, as shown in Table~\ref{tab:symbols:2}. Among all symbols, $\mathcal{N}$ is the only symbol associated with benign sender accounts.

Symbol $\mathcal{F}$ defines the transaction subspace of any future transaction sent from an adversarial account; the future transaction is defined w.r.t. the current state. \textsc{mpfuzz} instantiates symbol $\mathcal{F}$ to concrete transactions of nonce $m+1$, value $1$ Ether, Gas price $m+1$ wei, and any adversarial account $A*$. The instantiating pattern for symbol $\mathcal{F}$ is $tx\begin{bsmallmatrix}{A*} & {1}\\ {m+1} & {m+1}\end{bsmallmatrix}$. 

Symbol $\mathcal{P}$ defines the transaction subspace of any parent transaction from an adversarial account w.r.t. the current state. \textsc{mpfuzz} instantiates $\mathcal{P}$ to a transaction of Pattern $tx{\begin{reduce}\begin{bsmallmatrix}{A\geq{r}} & {1}\\ {1} & {[4,m]}\end{bsmallmatrix}\end{reduce}}$. Here, the transaction is fixed with a Gas price in the range $[4,m]$ wei, value at $1$ Ether, and nonce at $1$. 
{ 
The gas price of a future transaction ($\mathcal{F}$) is $m+1$ wei, which is higher than the price of a parent transaction ($\mathcal{P}$) in $[4,m]$ wei. The purpose is to ensure that a future transaction can evict any parent transaction during fuzzing.
}

Symbol $\mathcal{C}$ defines the transaction subspace of any adversarial child transaction w.r.t. the state. \textsc{mpfuzz} instantiates $\mathcal{C}$ to a transaction of Pattern $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$. The instantiated child transaction is fixed at Gas price of $m+1$

Symbol $\mathcal{O}$ defines the transaction subspace of any adversarial overdraft transaction w.r.t. state $st$. \textsc{mpfuzz} instantiates $\mathcal{O}$ to a transaction of Pattern $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m+1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$. Recall that all adversarial accounts have an initial balance of $m$ Ether.

Symbol $\mathcal{L}$ defines the transaction subspace of any adversarial latent-overdraft transaction w.r.t. state $st$. \textsc{mpfuzz} instantiates $\mathcal{L}$ to a transaction of Pattern $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m-1}\\ {\geq{}2} & {m+1}\end{bsmallmatrix}\end{reduce}}$. All adversarial accounts have an initial balance of $m$ Ether.

Symbol $\mathcal{R}$ defines the transaction subspace of any adversarial ``replacement'' transaction w.r.t., the state. Unlike the symbols above, the transactions under Symbol $\mathcal{R}$ must share the same sender and nonce with an existing transaction in the current state $st$. \textsc{mpfuzz} instantiates $\mathcal{R}$ to a transaction of Pattern $tx{\begin{reduce}\begin{bsmallmatrix}{A[1,r]} & {m-1}\\ {1} & {m+1}\end{bsmallmatrix}\end{reduce}}$. Here, we simplify the problem and only consider replacing the transaction with nonce $1$.


\begin{figure}[!bthp]
\centering
%\includegraphics[width=0.49\textwidth]{figures/tx-space.eps}
\includegraphics[width=0.49\textwidth]{figures/tx-space2.eps}
\caption{Symbols and transaction space reduction.}
\label{fig:opsymbols}
\end{figure}

Given that a concrete transaction in this work consists of four attributes, transactions are defined in a four-dimensional space. We visualize transaction symbols (with an incomplete view) in two two-dimensional spaces in Figure~\ref{fig:opsymbols}, that is, one of transaction sender and nonce and the other of sender and value. 
For each symbol, the figures depict the transaction subspace covered by the symbol (in white shapes of black lines) and the transaction pattern instantiated by \textsc{mpfuzz} under the symbol (in red lines or shapes). In our design, the instantiated transactions are a much {\it smaller subset} of the defining transaction space. 
For instance, given state $st$ of transactions sent from account $A_1,\dots,A_r$, 
transaction $tx{\begin{reduce}\begin{bsmallmatrix}{A_{r+1}} & {*}\\ {3} & {*}\end{bsmallmatrix}\end{reduce}}$
is within the defining space of symbol $\mathcal{F}$, but \textsc{mpfuzz} does not instantiate $\mathcal{F}$ by transaction $tx{\begin{reduce}\begin{bsmallmatrix}{A_{r+1}} & {*}\\ {3} & {*}\end{bsmallmatrix}\end{reduce}}$ (but instead to transactions $tx{\begin{reduce}\begin{bsmallmatrix}{A*} & {1}\\ {m+1} & {m+1}\end{bsmallmatrix}\end{reduce}}$).
%
The design rationale of transaction symbolization is deferred to Appendix~\ref{appdx:sec:sym:rationale}.

\vspace{-0.1in} \subsubsection{State Search Algorithm}

\input{text/lst14_fuzz.tex}

\noindent{\bf
Algorithm overview}:
We propose a stateful fuzzing algorithm, listed in Algorithm~\ref{alg:fuzz3}, to selectively explore the input space in a way that prioritizes new and promising mempool states towards triggering ADAMS oracle. 

The core data structure is a seed corpus or $sdb$ which stores a list of input-state pairs or seeds. Upon running the algorithm, the corpus maintains the mempool states covered so far by the algorithm execution.
The algorithm runs an outer loop that continues until the corpus is empty, or only the states of zero energy are left, or timeout. In each iteration, the algorithm retrieves the next seed from the corpus based on how promising the seed is in reaching a state triggering the oracle (a.k.a., the energy~\cite{DBLP:conf/uss/BaBMR22}). 
A seed consists of a symbolized input $ops$, which consists of transaction symbols, and a symbolized state $st$ reached by running a transaction sequence instantiated from the input $ops$ (Line~\ref{alg:fuzz2:next}). The algorithm runs an inner loop, in each iteration of which it mutates the input in the current seed ($\langle{}st, in\rangle{}$) and executes the mutated input against a reinitialized empty mempool, producing end state $st'$ (Line~\ref{alg:fuzz2:exec}). If the end state satisfies ADAMS conditions (i.e., the test oracle), it emits the mutated input-state pair $ops',st'$ as a newly found exploit. The algorithm further checks the feedback: The feedback is positive if the mutated input $ops'$ brings the mempool state $st'$ closer to triggering the test oracle than $st$. This entails mutated state $st'$ to be different from state $st$ (i.e., increased state coverage) and state $st'$ to achieve larger damage or lower attack cost. In case of positive feedback, the algorithm would add mutated input-state pair $ops',st'$ to the corpus. 

This algorithm assumes the mempool is deterministic. That is, given a seed $\langle{}ops, st\rangle{}$, running the same input $ops$ against an empty mempool multiple times always results in the same end state $st$. In practice, we generate inputs to avoid the non-deterministic behavior of real mempool implementations. 

The algorithm can be configured with initial seeds and input-mutation strategies. By default, we use one initial seed whose input fills up the mempool with normal transactions. The default input-mutation strategy is to append the current input with a newly generated transaction. 

\begin{algorithm}[h]
\caption{mutateExec(SymbolInput $ops$, SymbolState $st$)}
\small \label{alg:fuzz3:input}
%\hspace*{\algorithmicindent} \textbf{Input}: 
\begin{algorithmic}[1]
\State $ops'$=mutateSymbol($ops$);
\label{alg:fuzz3:input:1}
\State $st_c$=executeUnappended($ops, ops'$);
\label{alg:fuzz3:input:2}
\State $st_c'$=executeAppended($ops', st_c, st$);
\label{alg:fuzz3:input:3}
\State \Return $st_c'$
\end{algorithmic}
\end{algorithm}

\noindent{\bf 
Input mutation}:
Given a symbolized input $ops$ and symbolized state $st$, the mutation algorithm is to explore each ``slightly'' different input $ops'$ and its associated state $st'$, such that the next stage can find the inputs producing positive feedback.

Internally, the algorithm proceeds at two levels, that is, symbols and concrete value. Specifically, as shown in Algorithm~\ref{alg:fuzz3:input}, 1) it appends the symbolized input $ops$ with a previously untried symbol, generating the ``mutated'' symbolized input $ops'$ (Line~\ref{alg:fuzz3:input:1} in Algorithm~\ref{alg:fuzz3:input}). In this step, the algorithm tries different symbols in the following order: $\mathcal{P}, \mathcal{L}, \mathcal{C}$. 
2) It instantiates symbolized $ops'$ to a transaction sequence and executes the sequence in the tested mempool to obtain the concrete end state (Line~\ref{alg:fuzz3:input:2} in Algorithm~\ref{alg:fuzz3:input}). This step is necessary for instantiating and executing the mutation in the next step. Specifically, in this step, the algorithm instantiates symbolized input $ops$ to a concrete input $in_c$, which is a sequence of transactions. It then drives the transactions to a reinitialized mempool for execution. It returns the resulting concrete state $st_c$.
3) The algorithm instantiates the appended symbols under the context of the previous state $st$ and $st_c$. At last, it executes the appended transaction on mempool $st_c$ to obtain the concrete end state $st'_c$ under the mutated input (Line~\ref{alg:fuzz3:input:3} in Algorithm~\ref{alg:fuzz3:input}).

\noindent{\bf 
Mutation feedback}: We describe how mempool states are symbolized before presenting state-based feedback.
In \textsc{mpfuzz}, a symbolized state $st$ is a list of transaction symbols, ordered first partially as follows: $\mathcal{N}\preceq{}\mathcal{E}\preceq{}\mathcal{F}\preceq{}\{\mathcal{P},\mathcal{L},\mathcal{C}\}$. $\mathcal{E}$ refers to an empty slot. State slots of the same symbols are independently instantiated into transactions, except for $\mathcal{P}, \mathcal{C}, \mathcal{L}$. Child transactions (i.e., $\mathcal{C}, \mathcal{L}$) are appended to their parent transaction of the same sender (i.e., $\mathcal{P}$). Across different senders, symbols are ordered by the parent's GasPrice. For instance, suppose a mempool stores four concrete transactions, $tx\begin{bsmallmatrix}{A_1} & {*}\\ {1} & {4}\end{bsmallmatrix}$, $tx\begin{bsmallmatrix}{B} & {*}\\ {100} & {100}\end{bsmallmatrix}$, $tx\begin{bsmallmatrix}{A_2} & {*}\\ {1} & {5}\end{bsmallmatrix}$, $tx\begin{bsmallmatrix}{A_1} & {*}\\ {2} & {10001}\end{bsmallmatrix}$
, they are mapped to four symbols, $\mathcal{P}, \mathcal{F}, \mathcal{P}, \mathcal{C}$, and are further ordered in a symbolized state by $\mathcal{F}\mathcal{P}\mathcal{C}\mathcal{P}$.

In \textsc{mpfuzz}, the feedback of an input $ops'$ is based on the symbolized end state $st'$. Positive feedback on state $st'$ is determined conjunctively by two metrics: 1) State coverage that indicates state $st'$ is not covered in the corpus, and 2) state promising-ness that indicates how promising the current state is to reach a state satisfying bug oracles.

%{\fontsize{9.5pt}{9.5pt}\selectfont
\begin{eqnarray}
\nonumber
feedback(st',st,sdb) &=& st\_coverage(st',sdb)==1 \land{} 
\nonumber
\\ &&
st\_promising(st',st)==1 
\label{eqn:feedback}
\end{eqnarray}
%}

Specifically, state coverage is determined by straightforwardly comparing symbolized state $st'$, as an ordered list of symbols, with all the symbolized states in the corpus. For instance, state $\mathcal{F}\mathcal{P}\mathcal{C}\mathcal{P}$ is different from $\mathcal{F}\mathcal{P}\mathcal{P}\mathcal{C}$. This also implies concrete transaction sequence $tx{\begin{reduce}\begin{bsmallmatrix}{A_1} & {*}\\ {1} & {4}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{B} & {*}\\ {100} & {100}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{A_2} & {*}\\ {1} & {5}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{A_1} & {*}\\ {2} & {10001}\end{bsmallmatrix}\end{reduce}}$ is the same with $tx{\begin{reduce}\begin{bsmallmatrix}{A_1} & {*}\\ {1} & {4}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{B} & {*}\\ {100} & {100}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{A_2} & {*}\\ {1} & {6}\end{bsmallmatrix}\end{reduce}}$, $tx{\begin{reduce}\begin{bsmallmatrix}{A_1} & {*}\\ {2} & {10}\end{bsmallmatrix}\end{reduce}}$, as they are both mapped to the same symbolized state.

How promising a state $st'$ is (i.e., $st\_promising(st')$) is determined as follows: A mutated state $st'$ is more promising than an unmutated state $st$ if any one of the three conditions is met: 1) State $st'$ stores fewer normal transactions (under symbol $\mathcal{N}$) than state $st$, implying more transactions evicted and higher damage (i.e., $evict\_normal(st', st) = 1$). 
2) State $st'$ declines (speculatively) more incoming normal transactions than state $st$, also implying higher damage (i.e., $decline\_normal(st',st) = 1$). 
3) The total fees of adversarial transactions in state $st'$ are lower than those in state $st$, implying lower attack costs. 
We consider two forms of costs: concrete cost and symbolized cost. The former, denoted by $cost(st')$, is simply the total fees of adversarial transactions instantiated from a symbolized state $st'$. The latter, denoted by $opcost(st')$, optimistically estimates the cost of transactions in the current state $st'$ that contributes to a future state triggering test oracle. We will describe the symbolized cost next. Formally, state promising-ness is calculated by Equation~\ref{eqn:promising}.  

%{\fontsize{9.5pt}{9.5pt}\selectfont
\begin{eqnarray}
\nonumber
st\_promising(st',st) & = & evict\_normal(st',st) == 1 \lor{} 
\\ \nonumber & & 
decline\_normal(st',st) == 1 \lor{} 
\\ \nonumber & & 
cost(st') < cost(st) \lor{} 
\\ & & 
opcost(st') < opcost(st)
\label{eqn:promising}
\end{eqnarray}
%}

\noindent{\bf
Seed energy}: Recall that in \textsc{mpfuzz}, the next seed is selected from the corpus based on energy. By intuition, the energy of a state is determined based on how promising the state is in triggering the test oracle. In addition to the state promising-ness used in deciding feedback, state energy incorporates fuzz runtime information, such as how many times the state has been selected.

Specifically, the energy of a seed $\langle{}ops, st\rangle{}$ is determined by Equation~\ref{eqn:energy}.

\begin{eqnarray}
%\nonumber 
%b &=& 1- {m'}/{m}\\
Energy(in,st) &=& b / opcost(st)
\label{eqn:energy}
\end{eqnarray}

First, each seed in the corpus records how many times it has been mutated. The more symbols it has mutated in the past, the less energy the seed currently has and the lower priority it will be selected next. 
%In Equation~\ref{eqn:energy}, $b$ is one minus the ratio of the number of mutations in the past ($m'$) over the total number of possible mutations ($m$). 
$b$ can be configured differently to traverse the state tree differently.
In particular, breadth-first search (BFS) is by the following configuration: $b=1$ if at least one symbol has not been tried (for mutation) in the current seed. Otherwise, $b=0$. 

Second, %like in feedback, 
we use the symbolized cost to estimate how promising a state is and use it in seed energy. 

\noindent{\bf Estimate state cost}: When \textsc{mpfuzz} determines how promising a state is, it needs to look beyond the current state and into all possible descendant states. We propose a heuristic that optimistically estimates the descendant-state costs given a current state. The key intuition is the following: In Ethereum, the validity of a child transaction (under symbol $\mathcal{C}$) depends on its parent/ancestor transaction. Thus, even though a transaction in the current state is valid, the transaction can be ``turned'' into an invalid one in subsequent states. We thus attribute, optimistically, the cost of transaction $\mathcal{C}$ to value $1$, so that it is preferable to a parent transaction $\mathcal{P}$ in input mutation and seed selection, and turning $\mathcal{C}$ into an invalid one like $\mathcal{L}$ or $\mathcal{F}$ is also encouraged. The cost profiles used in \textsc{mpfuzz} are summarized in Table~\ref{tab:symbols:2}.

\vspace{-0.1in} \section{Found Exploits}
\label{sec:exploits}
\newcolumntype{C}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{2cm}}
\definecolor{darkolivegreen}{rgb}{0.33, 0.42, 0.18}
\definecolor{ferngreen}{rgb}{0.31, 0.47, 0.26}
\definecolor{forestgreen}{rgb}{0.0, 0.27, 0.13}

\begin{table*}[!htbp]
  \caption{ADAMS exploit patterns found by \textsc{mpfuzz} across Ethereum clients; $XT_{1-7}$ are eviction based, and $XT_{8-9}$ are locking based. $XT_{1-3}$ are known patterns in DETER~\cite{DBLP:conf/ccs/LiWT21}, while others are new. \xmark{} indicates the presence of a bug,  {\color{green} \cmark{}} indicates the fixing of a bug after our reporting, and \cmark{} indicates the fixing of a bug by previous works.}
  \label{tab:bug-report}
  \centering{\small
  \begin{tabularx}{0.85\textwidth}{ l|ccccccc|cX }
  & $XT_1$ &$XT_2$&$XT_3$&$XT_4$&$XT_{5}$&$XT_6$&$XT_7$ &$XT_8$&$XT_9$\\ \hline 
   \makecell{Geth $\geq{}v1.11.4$, { Flashbot $\le{}v1.11.5$ , bloXroute,} \\ {BSC $\le{}v1.3.8$, core-geth$\le{}v1.12.18$}} & \cmark{} & \cmark{} & & {\color{green}\cmark} & \xmark{} & \xmark{} &  &&\\ 
   \rowcolor{Gray} Geth $<v1.11.4$, { EigenPhi} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & && \\ 
   { go-opera $\le{}v1.1.3$} &  & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & && \\ 
   \rowcolor{Gray} Erigon $\le{}v2.42.0$ &  &  & & \xmark{} & & & &&\\
   Besu $\geq{}v22.7.4$ & \cmark{} & \xmark{} &  & \xmark{} &  & & &&\\ 
   \rowcolor{Gray} Besu $<v22.7.4$ &\xmark{} & \xmark{} &  & \xmark{} &  & & &&\\ 
   Nethermind $\geq{}v1.18.0$ & \cmark{} & &  & \xmark{} & & & {\color{green}\cmark} &&\\ 
   \rowcolor{Gray} Nethermind $<v1.18.0$& \xmark{} &  &  & \xmark{} &  &  & \xmark{} &&\\ 
   Reth $\geq{}v0.1.0-alpha.6$ &  &  &  & \xmark{} & & & & {\color{green} \cmark} &\\
   \rowcolor{Gray} Reth $<v0.1.0-alpha.6$ &  &  & &  & & & &\xmark&\\
   OpenEthereum $\le{}v3.3.5$ &  &  & & \xmark{} & & & &&\xmark
 \end{tabularx}}
\end{table*}

{  
We have run \textsc{mpfuzz} across a variety of Ethereum clients, including six leading execution-layer clients on the public-transaction path of Ethereum mainnet (Geth, Besu, Nethermind, Erigon, Reth, and OpenEthereum), three PBS clients (proposer-builder separation) on the mainnet's private-transaction and bundle path (Flashbot builder $v1.11.5$~\cite{me:flashbotbuilder}, EigenPhi builder~\cite{me:eigenphibuilder} and bloXroute builder-ws~\cite{me:bloXroutebuilder}), and the clients deployed on three operational Ethereum-like networks (BSC $v1.3.8$~\cite{me:bscclient} deployed on Binance Smart Chain, go-opera $v1.1.3$~\cite{me:goopera} on Fantom, and core-geth $v1.12.19$~\cite{me:coregeth} on Ethereum Classic). 

On the six public-transaction clients, \textsc{mpfuzz} leads to the discovery of $22$ bugs, as listed in Table~\ref{tab:bug-report}, including $7$ conforming to the known DETER attacks on clients of historical versions and $15$ new bugs on the clients of the latest versions. 

Other clients, including the three PBS clients and three clients on Ethereum-like networks, are mostly forks of the Geth clients except for minor code changes\footnote{For instance, go-opera adopts its own fix against $XT_1$ based on the fork of Geth $<v1.11.4$.}, and on them, \textsc{mpfuzz} discovered $13$ bugs of a similar nature to those found on Geth (of the historical and latest versions), as seen in Table~\ref{tab:bug-report}.

We describe the patterns of these bugs as follows.
}

\vspace{-0.1in} \subsection{Found Eviction Attacks}
\label{sec:foundevictionattacks}
\noindent{\bf 
Exploit $XT_1$: Direct eviction by future transactions}:
In this attack, given a mempool's initial state storing normal transactions, the attacker sends future transactions at high fees to evict the normal transactions. This exploit is essentially the DETER-X attack~\cite{DBLP:conf/ccs/LiWT21}.

In practice, Geth ($\leq{}v1.11.4$), Nethermind, Besu,{  and EigenPhi} are vulnerable under this exploit, as in Table~\ref{tab:bug-report}.

\noindent{\bf 
Exploit $XT_2$: Direct eviction by latent overdraft transactions}:
In this eviction attack, the attacker sends latent-overdraft transactions at high fees to evict the normal transactions initially stored in the target mempool. These transactions are sent from $k$ accounts, each of which sends $l$ transactions, denoted by $k\times{}l$. The intention is to evade the limit on the number of transactions per sender. The evasion increases the attacker cost from one pending transaction to multiple. 
This exploit is essentially the DETER-Z attack~\cite{DBLP:conf/ccs/LiWT21}.

In practice, Geth ($\leq{}v1.11.4$), Besu,{  
EigenPhi, and go-opera}
are found vulnerable under this exploit. 

\noindent{\bf 
Exploit $XT_3$: Compositional direct eviction} (by combining $XT_1$ and $XT_2$):
In some Ethereum clients, notably Geth, the limit on the number of transactions per sender is triggered under the condition that the mempool stores enough pending transactions (e.g., more than 5120 transactions in Geth). 
This eviction attack combines $XT_1$ and $XT_2$ to avoid triggering the condition and evade the protection. It works by maximizing the eviction of mempool under $XT_1$ until it is about to trigger the condition. It then conducts $XT_2$ by sending latent overdraft transactions under one sender, that is, $1\times{}l$. Compared to $XT_2$, the combined exploit $XT_3$ achieves lower costs.

In practice, Geth ($\leq{}v1.11.4$) is vulnerable under this exploit where its mempool of capacity of 6144 slots triggers the limit of 16 transactions per sender when there are more than 5120 pending transactions. That is, $XT_3$ is configured with $l=5120$.
Other clients including{  
EigenPhi and go-opera} are also vulnerable.

\noindent{\bf 
Exploit $XT_4$: Indirect eviction by valid-turned-overdraft transactions}: 
This eviction attack works in two steps: 1) The attacker first sends valid transactions at high fees to evict normal transactions initially stored in the mempool. These transactions are sent from $k$ accounts, each of which sends $l$ transactions. 2) She then sends $k$ transactions; each of the transactions is of nonce $1$, at a high fee, of high value $v_1$, and from the same $k$ accounts in Step 1). The transactions would replace the transaction of the same sender and nonce sent in Step 1). Once the replacement is finished, they turn their child transactions into latent overdraft. Specifically, if a sender's balance is $bal$ and the Ether value of transaction of nonce 2 is $v_2$, then $v_1$ is carefully crafted to enable turned latent overdraft, that is, $v_1<bal$ and $v_1+v_2>bal$.

In practice, many clients are found vulnerable under this exploit, including Geth $<v1.11.4$, Erigon, Besu, Nethermind, OpenEthereum,{  
EigenPhi, and go-opera}. 

\noindent{\bf 
Exploit $XT_5$: Indirect eviction by valid-turned-future transactions}:
This eviction attack works in two steps: 1) The attacker first sends valid transactions at high fees to evict normal transactions initially stored in the mempool. These transactions are sent by $k\times{}l$, that is, from $k$ accounts, each with $l$ transactions. For each sender, the transaction of nonce 1 has a fee, say $f_1$, slightly lower than the transactions of other nonces, that is, $f_1<f_2$. 
2) She then sends $k$ transactions; each of the transactions is from a distinct sender from those used in Step 1) and of fee $f'$ that $f_1<f'<f_2$. The intent is that the $k$ transactions in Step 2) evict the transactions of nonce $1$ sent in Step 1), turning other child transactions sent in Step 1) into future transactions. 

\noindent{\bf 
Exploit $XT_6$: Compositional indirect eviction} (by multi-round valid-turned-future transactions): 
{
This exploit is an adaptive attack to the Geth $\geq{}v1.11.4$. Geth $\geq{}v1.11.4$ is patched against $XT_{1-2}$ and adopts the following admission policies: The mempool of $m'=6144$ slots admits up to $py_1'=1024$ future transactions. When containing more than $py_3'=5120$ pending transactions, the mempool starts to limit that no more than $py_2'=16$ pending transactions from the same sender can be admitted.

Exploit $XT_6$ works in three steps: 1) it first evicts the initial mempool of normal transactions with $m'/py_2'=384$ sequences, each of $16$ transactions sent from one unique sender, 2) it then sends $py_1'/py_2'=64$ transactions to evict the parent transactions and creates $py_1'=1024$ future transactions in the mempool, 3) it sends one sequence of $5120$ transactions from one sender to evict the normal transactions sent in Step 1), and 4) it sends one transaction to evict the parent transaction in Step 3, leaving the mempool of just one valid transaction. Step 3) can succeed because the precondition (w.r.t. $py_3'=5120$) of limiting transactions of the same sender does not hold.}

In practice, Geth of all versions and the Geth forks, including 
{  
Flashbot, bloXroute, BSC, and Ethereum Classic} are found vulnerable under $XT_6$.

\noindent{\bf 
Exploit $XT_7$: Reversible evictions}: 
Suppose a mempool of state $st$ admits an arriving transaction $tx$ by evicting an existing transaction $tx'$, transitioning its state to $st'$. A mempool is reversible if one sends $tx'$ to state $st'$, and the mempool admits $tx'$ by evicting $tx$, transitioning its state back to $st$.

The mempool on Nethermind $<v1.18.0$ can be reversible: Minimally, suppose a two-slot mempool stores $tx_1$ of low fee from one sender and $tx_2$ of medium fee from another sender $A2$ and receives $tx_3$ as a child of $tx_1$ and of high fee. For instance, $tx_1\begin{bsmallmatrix}{A} & {1}\\ {1} & {1}\end{bsmallmatrix}$, $tx_2\begin{bsmallmatrix}{B} & {1}\\ {1} & {3}\end{bsmallmatrix}$,  $tx_3\begin{bsmallmatrix}{A} & {1}\\ {2} & {5}\end{bsmallmatrix}$. The Nethermind $<v1.18.0$ mempool would admit $tx_3$ and evict $tx_2$. After that, if one resends the evicted $tx_2$ back to the mempool storing $tx_1$ and $tx_3$, the Nethermind  $<v1.18.0$ mempool would admit $tx_2$ and evict $tx_3$, looping back to its initial state.

An attacker observing reversible mempool mounts Exploit $XT_7$ to evict the mempool while bringing down attack costs. On Nethermind $<v1.18.0$, the attack works in two steps: 1) She first sends $k$ transaction sequences from $k$ senders,\footnote{Nethermind does not limit transactions per sender, thus $k=1$ in actual attacks.} each of $l$ transactions (i.e., $k\times{}l$). In each $l$-transaction sequence, the nonce-$1$ transaction has a low fee, say $f_1$, while all its child transactions are of high fees, evicting normal transactions initially stored in the mempool. 2) The attacker sends $k\times(l-1)$ transactions from $k\times(l-1)$ new senders, all with fees slightly higher than $f_1$. The mempool would admit these transactions to the mempool by evicting all child transactions sent in Step 1), bringing down the attack costs.

%\input{text/exploit3.tex}

\vspace{-0.1in} \subsection{Found Locking Attacks}

\noindent{\bf
Exploit $XT_8$: Locking FIFQ}: Certain mempool design prohibits eviction by admitting transactions as a FIFQ. Transactions are admitted to a mempool only when there are empty slots. A full mempool always declines an arriving transaction. In practice, Reth $v0.1.0-alpha.4$ adopts the FIFQ mempool design.

While a FIFQ mempool can not be vulnerable to eviction attacks, it can be easily locked by Exploit $XT_8$ as follows: Whenever the attacker observes an empty slot present in the mempool, she sends a pending transaction of a minimally necessary fee to occupy the slot. Any transactions that arrive after will encounter a full mempool and are declined.


\noindent{\bf
Exploit $XT_9$: Locking mempool of no turning}: Because of the risk of evicting a parent transaction that could lead to turning, certain mempool is designed to restrict eviction victims to child transactions; that is, only the transaction of maximal nonce under a given sender can be evicted. For instance, given an arriving transaction $tx$, the OpenEthereum mempool finds an existing child transaction $tx'$ with a lower fee than $tx$ and evicts it to admit $tx$. 

In Exploit $XT_9$, the attacker observes empty slots in the mempool (e.g., created by arriving blocks) and sends the same number of transactions to occupy them. The transactions are sent from one account where the child transaction has a higher fee $f_1$ than normal transactions, while all its parent transactions have minimal fees. A normal transaction that arrives subsequently is declined because $f_1$ is higher than the fee of a normal transaction. Because each of its parent transactions has a low fee, the mempool is locked at a low cost.

\vspace{-0.1in} \subsection{Evaluation of Found Turning Exploits}
\label{sec:evaluate}
\label{sec:evaluate:turning}

This and next subsections show the evaluation of turning attacks and locking attacks, and due to the space limit, the evaluation of other ADAMS attacks is deferred to Appendix~\ref{appdx:sec:eval:locking} and Appendix~\ref{appdx:sec:additional-attack-evaluation}.

We design experiments to measure the success of ADAMS attacks in real Ethereum networks.

\vspace{-0.1in} \subsubsection{Evaluation in Testnet}
\label{sec:eval:multi:turning}

\ignore{
\begin{center}
\fbox{\parbox{0.90\linewidth}{
RQ1. What's the success rate and attack cost in mounting a turning/eviction attack against a testnet? Particularly, can the crafted transactions in a turning attack be propagated through the testnet?
}}\end{center}
}

\label{sec:evaluate:testnet}
\noindent{\bf Experimental settings}: 
We set up our experiment platform by connecting the attacker node to the Goerli testnet. The attacker node runs an instrumented Geth client at
the execution layer which sends crafted transactions to the testnet.

\ignore{
\begin{figure}[!bthp]
\centering
%\includegraphics[width=0.375\textwidth]{figures/exp-setup.eps}
\includegraphics[width=0.425\textwidth]{figures/exp-setup5.eps}
\caption{Experimental setup for evaluation of turning attacks on Goerli testnet}
\label{fig:exp:setup5}
\end{figure}
}

To monitor transaction propagation, we launch an independent supernode (called measurement node) in the same testnet. The measurement node runs a reconfigured Geth client where the limit of peers/neighbors is removed and the measurement node can connect to as many neighbors as possible, hence a super node. 
%As shown in Figure~\ref{fig:exp:setup5}, 
The measurement node is not (directly) connected to the attacker node. When setting up our experiments, we ran the measurement node in Goerli for seven days and found the node is stabilized at $290$ neighbors. 

\ignore{
\begin{figure*}[!htbp]
 \centering
  \subfloat[Transaction propagation in six messages]{%
 \includegraphics[width=0.295\textwidth]{figures/propagatino_rinkeby_by_nonce.eps}
 \label{fig:testnet:rinkeby_ed4_percentage}}
  \subfloat[Transaction propagation in two messages]{%
 \includegraphics[width=0.295\textwidth]{figures/propagatino_rinkeby_by_nonce_1msg.eps}
 \label{fig:testnet:rinkeby_ed4_percentage_1msg}}
 % \subfloat[Etherscan screenshot of the blocks generated during the attack on Goerli (txs in two messages)]{%
 %\includegraphics[width=0.325\textwidth]{figures/attack-screenshot3.eps}
  \subfloat[Etherscan screenshot of the blocks generated during the attack on Goerli (txs in six messages)]{%
 %\includegraphics[width=0.325\textwidth]{figures/ED4-attack-screenshot-bigMempool.eps}
 \includegraphics[width=0.325\textwidth]{figures/ED4-post-merge-testnet2.eps}
 \label{fig:testnet:rinkeby_ed4}
  }%
 \caption{Mounting $XT_4$ attacks on Goerli: Emptying blocks and propagating malicious transactions to the entire network.}
\end{figure*}

\begin{table}[!htbp]
  \caption{Types of transactions included in the four blocks during the attack in Figure~\ref{fig:testnet:rinkeby_ed4}. `\# private tx' means the number of private transactions.}
  \label{tab:privatetransactions2}
  \centering{\small
  \begin{tabularx}{0.425\textwidth}{ |l|X|X|X| }
  \hline
  \# block & \# private txs & \# public txs & \# attack txs \\ \hline 
  $8040010$ & $5$ & $0$ & $384$ \\ \hline 
  $8040009$ & $78$ & $4$ & $384$ \\ \hline 
  $8040008$ & $1$ & $0$ & $384$ \\ \hline 
  $8040007$ & $5$ & $0$ & $384$ \\ \hline 
\end{tabularx}
}
\end{table}
}

\begin{figure}
  \begin{minipage}[b]{.5\linewidth}
  \centering
  \subfloat[Propagation in six messages]{\label{fig:testnet:rinkeby_ed4_percentage}\includegraphics[width=.93\linewidth]{figures/propagatino_rinkeby_by_nonce.eps}}
  \end{minipage}%
  \begin{minipage}[b]{.5\linewidth}
  \centering
  \subfloat[][Propagation in two messages]{\label{fig:testnet:rinkeby_ed4_percentage_1msg}\includegraphics[width=.93\linewidth]{figures/propagatino_rinkeby_by_nonce_1msg.eps}}
  \end{minipage}\par\medskip
  \centering
  \subfloat[Etherscan screenshot of the blocks generated during the attack on Goerli (txs in six messages)]{\label{fig:testnet:rinkeby_ed4}\includegraphics[width=0.33\textwidth]{figures/ED4-post-merge-testnet2.eps}}
  \caption{Mounting $XT_4$ attacks on Goerli: Emptying blocks and propagating malicious transactions to the entire network.}

\end{figure}

\noindent{\bf Experiment results}: The instrumented measurement node is able to log the received messages from different neighbors; these messages include those of transactions and of transaction hashes. The measurement node could receive the same transaction from different neighbors, and the log stores the transaction-neighbor pairs. We started logging the received messages one month before the experiment.

To do an experiment, we make the attacker node send $XT_4$ transactions using $384$ accounts. Each account sends $16$ valid pending transactions, followed by a replacement transaction. In total, the attacker node sends $6144$ valid transactions and $384$ replacement transactions. The Gas prices of the valid and replacement transactions are set to be $8$ Gwei and $130$ Gwei, respectively. 
In one setting, we split the $6528$ transactions into six messages (i.e., the first five being $1229$ transactions each and the last one with $384$ transactions). We send these messages in order and wait for $1.5$ seconds between two consecutive messages. For comparison, in another setting, we send the $6144$ valid transactions in one message and the $384$ replacement transactions in another message. Finally, we wrap up the experiment by waiting after the attacker node sends all messages and all replacement transactions are included in the blockchain. 
We then turn off the measurement node's logging and search for the presence of all $6528$ transactions across neighbor nodes in the log. Given a transaction nonce, we report the percentage of neighbor nodes in the testnet that have propagated it to the measurement node.

\ignore{
\begin{table}[!htbp]
      \caption{Types of transactions included in the four blocks during the attack in Figure~\ref{fig:testnet:rinkeby_ed4}. `\# private tx' means the number of private transactions.}
      \label{tab:privatetransactions}
      \centering{\small
      \begin{tabularx}{0.425\textwidth}{ |l|X|X|X| }
      \hline
      \# block & \# private txs & \# public txs & \# attack txs \\ \hline 
      $8040010$ & $5$ & $0$ & $384$ \\ \hline 
      $8040009$ & $78$ & $4$ & $384$ \\ \hline 
      $8040008$ & $1$ & $0$ & $384$ \\ \hline 
      $8040007$ & $5$ & $0$ & $384$ \\ \hline 
    \end{tabularx}
    }
\end{table}
}


We run experiments of six-message and two-message propagation, repeat each experiment by $3$ times, and report the average result of node percentage in Figure~\ref{fig:testnet:rinkeby_ed4_percentage} and Figure~\ref{fig:testnet:rinkeby_ed4_percentage_1msg}. Figure~\ref{fig:testnet:rinkeby_ed4_percentage} shows the transaction propagation with six messages. More than 90\% of the testnet nodes have received all of the $15$ valid transactions in a sequence and the replacement transactions. The only exception is the relatively low percentage for the $16$-th transaction of the maximal nonce. By comparison, when sending the transactions in two messages, the propagation fails as shown in Figure~\ref{fig:testnet:rinkeby_ed4_percentage_1msg} where nodes did not propagate any transaction of nonce larger than $5$. 

Additionally, Figure~\ref{fig:testnet:rinkeby_ed4} shows the generated blocks in the experiment propagating six messages. We took the screenshot from \url{etherscan.io} and labeled it in red with information regarding the attack. Before the attack begins, the Goerli testnet normally utilizes $24-47\%$ of the Gas in a block. For ethics, our attacks are short (lasting four blocks). 

Right after the launch of the attack, in block $8040007$, the Gas used by normal transactions drops to $3.19\%$ and the Gas used by adversarial transactions (denoted by red bars in Figure~\ref{fig:testnet:rinkeby_ed4}) is $26.88\%$. The included adversarial transactions are $384$ replacement transactions sent in the second round of $XT_4$. The $6144-384=5760$ child transactions sent in the first round are not included in the block. Other blocks during the attack, namely $8040008$ and $8040010$, are similar. In the third block $8040009$, $73.1\%$ Gas is spent on including $82$ normal transactions.% as shown in Table~\ref{tab:privatetransactions} not sent by our attacker node. 
To explain it, we inspect the raw history of transactions arriving at and logged by our measurement supernode and found that out of the $82$ included normal transactions, only $4$ are present in the log, implying the other $78$ normal transactions are private ones that were not broadcast to the measurement node. 
%Furthermore, the private mempool in today's Ethereum clients~\cite{me:PBS:builder} has a capability of no limit, which, while being feasible under today's low private-transaction workloads, can cause resource-exhaustion vulnerability as discussed in Appendix \S~\ref{sec:privatepool}.
%Overall, of the four blocks during the attack, the average Gas utilization per block drops to $19.97\%$, while the pre-attack utilization is consistently above $24.9\%$.
%
Notice that our attacks require no discovery of critical nodes as needed in~\cite{DBLP:conf/ccs/LiWT21}. 

\vspace{-0.1in} \subsection{Evaluation of Found Locking Exploits}
\label{sec:eval:locking:xt8a}
Given Exploit $XT_8$ found on Reth, we manually extended it to two actual exploits on unmodified Reth's mempool, $XT_{8a}$, and $XT_{8b}$. Due to space limit, this subsection focuses on the evaluation of $XT_{8a}$ and defers the evaluation of $XT_{8b}$ and $XT_9$ to Appendix~\ref{appdx:sec:eval:locking}.

\vspace{-0.1in} \subsubsection{Exploit Extension}

\noindent{\bf Mempool in Reth $v0.1.0-alpha.4$}: Recall that the mempool is a FIFO queue: Any transaction residential in the mempool is never evicted, no matter how high an arriving transaction's fee is. Besides, when there is an empty slot in its mempool, it requires that the transaction admitted must have fees higher than the latest block's base fee. 

\noindent{\bf 
Actual exploit $XT_{8a}$}: In $XT_8$, the attack cost increases with the block base fee. We manually propose a method to decrease the block base fee in Ethereum by mounting an eviction attack on the previous block. Specifically, in Ethereum (after EIP1559), given a recently produced block $i$, the base block fee of block $i+1$ is calculated dynamically as follows: 

{\fontsize{9.2pt}{9.2pt}\selectfont
\begin{eqnarray}
BaseFee(i+1) &=& BaseFee(i) * [\frac{7}{8} + \frac{1}{4} * \frac{GasUsed(i)}{BlockLimit}]
\end{eqnarray}
}

Therefore, if an eviction attack can persistently lower the Gas utilization of recent blocks, the current block fees can be reduced, which decreases the costs of locking attacks on the current block. In Exploit $XT_{8a}$, we mount a series of eviction attacks first and then a locking attack against the Reth node. 

Specifically, suppose in a network of a Reth node and a block validator node, the $XT_{8a}$ attacker first keeps sending eviction attacks directly to the validator node for several consecutive blocks. When observing the block base fees drop sufficiently, the attacker mounts the regular locking attack $XT_{8}$ against the Reth node.

\vspace{-0.1in} \subsubsection{Attack Evaluation on Reth}

\noindent{\bf Experimental settings}: 
We set up an experiment platform for evaluating locking attacks, on which an attacker node is connected to a victim non-validator node, which is also connected to a workload generator node and a victim validator node. The attacker node also maintains a direct connection to the victim validator. The network topology is depicted in Figure~\ref{fig:exp:setup3}. The non-validator node runs the Geth $v1.11.4$ client.

\begin{figure}[!bthp]
\centering
\includegraphics[width=0.425\textwidth]{figures/exp-setup3.eps}
\caption{Experimental setup for locking attacks on Reth}
\label{fig:exp:setup3}
\end{figure}



%\begin{figure}[!ht]
%  \centering
%  \subfloat[Attacks of $XT_{8a}$]{%
%   \includegraphics[width=0.25\textwidth]{figures/reth-locking.eps}
%  \label{fig:reth-lock}}
%  \subfloat[Attacks of $XT_{8b}$]{%
%    \includegraphics[width=0.22\textwidth]{figures/reth-sideeffect-%locking.eps}
%    \label{fig:side-effect-locking}}%
%   \caption{Evaluation of locking attacks on Reth}%
%\end{figure}
\label{sec:evaluate:locking}
\begin{figure}[!htb]
  \centering
  \includegraphics[clip,width=0.8\columnwidth]{figures/reth-locking.eps}%
  \caption{Evaluation of locking attack $XT_{8a}$ on Reth}%
  \label{fig:reth-lock}
\end{figure}

\noindent{\bf 
Evaluation of $XT_{8a}$}: To evaluate $XT_{8a}$, we set up the workload generator that sends normal transactions to the validator Geth node. The non-validator Reth node has not yet joined the network. We let the attacker node first send eviction attacks ($XT_6$) directly to the victim validator for $35$ consecutive blocks until it observes the block base fees drop sufficiently to $1$ Gwei, which occurs at the $45$-th in our experiment. The Reth node then joins the network with an empty mempool. The attacker node mounts a locking attack $XT_8$ with transactions of price $5$ Gwei to occupy the Reth node's mempool.

We report the total fees of normal transactions included in the blocks – the lower the fees are, the more successful the locking attack is. We also report the adversarial transaction fees as the attack cost shown in Figure~\ref{fig:reth-lock}. When the locking attack begins at the $45$-th block, the normal transaction fees increase because of the empty mempool on the Reth node which accepts some normal transactions in addition to the adversarial locking transactions. Then, after three blocks, the normal transaction fees quickly drop to near-zero Ether, showing the success of locking attacks. Interestingly, unlike the eviction attacks that cause low Gas utilization per block, the locking attacks just reduce the total Ether fees without reducing Gas utilization (i.e., the blocks produced under locking attacks from height $45$ to $60$ use the Gas of almost $100\%$ block limit as shown in Figure~\ref{fig:reth-gas}). Due to the high Gas utilization, block base fees keep increasing during the locking attack. When reaching the $60$-th block, the base fee is higher than the maximal transaction price tolerable by the attacker. In our experiment, the locking attacker stops at $60$-th block, and the normal transaction fees immediately recover to the ``normal'' level. In practice, the attacker can repeat sending eviction attacks to reduce the base fee before mounting the locking attack again.

\vspace{-0.1in} \section{Evaluation of \textsc{mpfuzz}}
\label{sec:eval:fuzz}

\vspace{-0.1in} \subsection{Performance}
\noindent{\bf 
Preliminary of GoFuzz}:
Upon each fuzzing iteration, GoFuzz~\cite{me:gofuzz} generates a bit-string of variable length, feeds it to our fuzzer code, and receives from our fuzzer a binary value of feedback, be either positive or negative. The GoFuzz further checks if this run increases the code coverage in the Geth client (as will be described, our fuzzer invokes functions in Geth's \texttt{txpool}). If the feedback is positive and code coverage increases, GoFuzz adds the current bit-string to the seeds before running into the next iteration. 

\noindent{\bf Baseline B1: Stateless fuzzer}. We implement a stateless fuzzer in the GoFuzz framework described above. 1) Given a bit string generated by GoFuzz, our fuzzer code parses it into a sequence of transactions; the length of the sequence depends on the length of the bit string. It skips a bitstring that is too short. 2) The fuzzer then sets up and initializes a Geth \texttt{txpool} instance with $m$ normal transactions, each sent from a distinct account, of nonce $1$, of value $1$ Ether (lower than the account balance), and of Gas price $3$ wei. 3) The fuzzer sends the transaction sequence to the initialized mempool for execution. 4) It checks the mempool state after execution: If the eviction-based test oracle (Equations~\ref{eqn:adams:evict:1}, ~\ref{eqn:adams:evict:2} and ~\ref{eqn:adams:evict:3}) is met, it emits the current transaction sequence as an exploit. 

\noindent{\bf Baseline B2: Concrete-state-coverage fuzzer}. We also build the second baseline, a mempool fuzzer that takes concrete state coverage as feedback. Specifically, in each iteration, the fuzzer appends a new transaction to the current transaction sequence. Given the $m$-slot mempool, the fuzzer tries $m$ values for senders, $m$ values for nonces, $m$ values for Gas price, and $m$ values for Ether amount. After sending the current transaction sequence to the mempool, it sorts the transactions in the mempool by senders and nonces. It then hashes the sorted transactions in the mempool and checks the presence of the hash digest in the seeds. If no hash exists, the current transaction sequence would increase the concrete-state coverage and is inserted to the corpus. The corpus is a FIFO queue where the seed inserted earlier has high priority to be de-queued.

\noindent{\bf Baseline B3: Invalid-tx energy fuzzer}. 
Baseline B3  is similar to B2 except that it uses as the energy the number of invalid transactions on a mempool state. The seed with more invalid transactions in the mempool has higher energy or priority to be selected for the next round of fuzzing.


{  
\noindent{\bf Baseline B4: feedback of no promising states}:  We design Baseline B4 for an ablation study on the effectiveness of using promising states as feedback in improving fuzzing performance. B4 is the same with \textsc{mpfuzz} except that it removes the state promising-ness from its feedback. Specifically, the feedback formula in B4 includes only state coverage ($st\_coverage$) and excludes state promisingness ($st\_promising$ as in Equation~\ref{eqn:feedback}). 
%In the case of two seeds of the same $st\_coverage$(WWW), B4 breaks even by using a FIFO strategy: the seed that was admitted to the corpus earlier or whose last time of being selected is earlier has the higher priority being selected this time.
}

We implement Baseline B1 in Go/GoFuzz and implement B2, B3 and B4 in Python.
%
We use a test oracle that can detect DETER attacks, that is, the number of invalid transactions in a mempool state equal $m-1$. 

{  
\label{sec:mut:setting}
\noindent{\bf Experimental settings of fuzzing}: 
We run the three baselines and \textsc{mpfuzz} against a MUT in a Geth client reconfigured under two settings: A small setting where the mempool is resized to $6$ slots $m=6$ and all fuzzers run for two hours (if test oracle is not triggered), and a medium setting where $m=16$ and fuzzers run for $16$ hours. The fuzzing experiments are run on a local machine with an Intel i7-7700k CPU of $4$ cores and $64$ GB RAM.
}

\begin{table}[!htbp] %force in current page, disable float.
\caption{Fuzzing Geth $v1.11.3$'s mempool (in minutes) by different approaches to detect Exploit $XT_3$.}
\label{tab:vs:baselines}
\centering{\footnotesize
%p{1.5cm}
\begin{tabularx}{0.475\textwidth}{ |X|c|c|c|c|c| }
  \hline
Settings & B1 & B2  & B3 & B4&\textsc{mpfuzz} \\ \hline
$6$slot-$2$h & Timeout & $54$ & $8$ &$1.22$ &$0.03$ 
\\ \hline
$16$slot-$16$h & Timeout & Timeout & $447$ & Timeout & $0.06$ 
\\ \hline
\end{tabularx}
}
\end{table}

\noindent{\bf
Results}: Table~\ref{tab:vs:baselines} reports the results under the small and medium MUT settings. For the small MUT of $6$ slots, Bbaseline B1 cannot find any DETER attack in two hours, B2 can find Exploit $XT_3$ in 54 minutes, B3 finds Exploit $XT_3$ in $8$ minutes, and { B4 in $1.22$ minutes}. By contrast, \textsc{mpfuzz} finds the same exploit ($XT_3$) in $0.11$ minutes.

For the medium setting, with $6$ slots,  baselines B1, B2, and B4 cannot find any DETER exploit in $16$ hours, and B3 can find Exploit $XT_3$ in $7.4$ hours. By contrast, \textsc{mpfuzz} finds the same exploit in under a minute.

%\begin{figure}[!ht]
%  \centering
%  \includegraphics[width=0.25\textwidth]{figures/fuzz-comparison1.eps}
%  \caption{\textsc{mpfuzz} on different clients: Number of found exploits on 16-slot mempool in 16 %hours.}%
%  \label{fig:exploits-found}
%\end{figure}

The evaluation on different clients is in Appendix~\ref{appdx:sec:mpfuzzeval:acrossclients}.

{ 
\vspace{-0.1in} \subsection{True/False Positive Rates}
\label{sec:falsepositives}

This section evaluates the true/false positives of the short exploits found by \textsc{mpfuzz}. 
%
Recall that \textsc{mpfuzz} runs against a small mempool (MUT) and may introduce false positives, that is, the exploits that satisfy bug oracles in MUT but do not in the actual larger mempool. We formally define true and false positives as follows: 

\begin{definition}[TP/FP exploits]
Consider a short exploit found by \textsc{mpfuzz} on a MUT, 
$\langle{}st_0, dc_0\rangle{}, ops \Rightarrow{}\langle{}st_n, dc_n\rangle{}$, and a (manually) extended exploit on an actual mempool, $\langle{}st_0', dc_0', ops' \Rightarrow{}\langle{}st_n', dc_n'\rangle{}$.

The pair of exploits constitute a true positive eviction attack w.r.t. $\epsilon$ ($\lambda$), if.f.
$st_0\cap{}st_n = \emptyset \land{} asym_E(st_0, ops) < \epsilon \land{}\  st_0'\cap{}st_n' = \emptyset  \land{} asym_E(st_0', ops') < \epsilon$ .

The pair of exploits constitute a false positive eviction attack w.r.t. $\epsilon$ ($\lambda$), if.f. 
$st_0\cap{}st_n = \emptyset \land{} asym_E(st_0, ops) < \epsilon \land{}\  (st_0'\cap{}st_n' \neq{} \emptyset  \lor{}  asym_E(st_0', ops') > \epsilon)$.

\end{definition}

True/false positives on locking attacks can be similarly defined from bug-oracle definitions~\ref{def:oracle:evict} and~\ref{def:oracle:lock}.

We evaluate the false positives of the exploits found by \textsc{mpfuzz} under varying $\epsilon$ and $\lambda$. Specifically, we design a two-step experiment: First, given a MUT, we run \textsc{mpfuzz} with varying $\epsilon$ (and $\lambda$). Increasing $\epsilon$ allows \textsc{mpfuzz} to find more short exploits; for each distinct short exploit, we manually extend it to an actual exploit. Second, we evaluate the extended exploits on an actual mempool (in the same local experimental setting as described in \S~\ref{appdx:sec:eval:local:1} and \S~\ref{appdx:sec:eval:local:2}). 

\begin{table}[!htbp]
  \caption{True/false positives (TP/FP) of eviction and locking attacks discovered with varying $\epsilon$ and $\lambda$. \cmark means satisfied.}
  \label{tab:fp:epsilon-attack}
  \centering{\footnotesize
  \begin{tabularx}{0.49\textwidth}{ |X|l|l|l|l|l|l| }
  \hline
  Exploit & $\epsilon$ &\multicolumn{2}{c|}{$m=16$ (MUT)}&\multicolumn{2}{c|}{Default $m$} & TP? \\ \cline{3-6} 
  &  & Eq.~\ref{eqn:adams:evict:1} & $asym_E$ & Eq.~\ref{eqn:adams:evict:1} & $asym_E'$&\\ \hline 
 Geth-$XT_1$ & $10^{-4}$ & \cmark & $0$ & \cmark & $0$ & \cmark \\ \hline
 Geth-$XT_3$ & $.09$ & \cmark & $0.083$ & \cmark & $0.0002$ & \cmark \\ \hline
 Geth-$XT_6$ & $.125$ & \cmark &$0.125$ & \cmark & $0.0003$ & \cmark \\ \hline
 Geth-$XT_2$ & $0.2$ & \cmark & $0.167$ & \cmark & $0.0698$ & \cmark \\ \hline
 Geth-$XT_4$ & $0.23$ & \cmark &$0.208$ & \cmark & $0.0768$& \cmark \\ \hline 
 Geth-$XT_5$  & $0.23$ & \cmark &$0.208$ & \cmark & $0.0768$& \cmark \\ \hline
 Nethermind-$XT_1$ & $10^{-4}$ & \cmark & $0$ & \cmark & $0$ & \cmark \\ \hline
 Nethermind-$XT_4$ & $0.11$& \cmark &$0.104$ & \cmark  & $0.0008$ & \cmark \\ \hline 
 Nethermind-$XT_7$  & $0.36$ & \cmark & $0.355$ & \cmark & $0.0012$ & \cmark \\ \hline
 Besu-$XT_2$ & $0.2$ & \cmark & $.167$ & \cmark & $0.0754$ & \cmark \\ \hline
 Besu-$XT_4$ & $0.23$ & \cmark & $.208$ & \cmark & $0.0083$ & \cmark \\ \hline
 Erigon-$XT_4$ & $0.23$ & \cmark & $0.208$ & \cmark & $0.0894$ & \cmark \\ 
\hline
\hline
  Exploit & $\lambda$ &\multicolumn{2}{c|}{$m=16$ (MUT)}&\multicolumn{2}{c|}{Default $m$} & TP? \\ \cline{3-6} 
  &  & Eq.~\ref{eqn:adams:decline:1} & $asym_D$ & Eq.~\ref{eqn:adams:decline:1} & $asym_D'$ &\\ \hline 
 Reth-$XT_8$ & $0.34$ & \cmark & $0.34$ & \cmark & $0.015$ & \cmark \\ \hline
 OpenEthereum-$XT_9$ & $0.46$ & \cmark & $0.46$ & \cmark & $0.0439$ & \cmark \\ \hline
\end{tabularx}
}
\end{table}

Table~\ref{tab:fp:epsilon-attack} presents the details of exploits discovered by \textsc{mpfuzz}. For instance, when setting $epsilon$ at $0.0001$ to find eviction attacks on Geth, \textsc{mpfuzz} discovered one short exploit $XT_1$ with $asym_E=0$ on MUT, which can be extended to an actual exploit on Geth mempool (of $m=6144$) with $asym_E'=0<0.0001=\epsilon$. This makes it a true positive (marked by \cmark in the table). Increasing $\epsilon$ to $0.23$ leads to discovering all six exploits $XT_{1-6}$ on Geth. All these exploits are true positives. The table also includes the results of eviction exploits found on other clients and locking exploits.
Overall, the true-positive rate of \textsc{mpfuzz} remains at $100\%$ for $\epsilon \leq{} 0.36$ and for $\lambda \leq{} 0.46$ across Ethereum clients.
}

\vspace{-0.1in} \section{Discussions}
\vspace{-0.1in}

{  
\noindent{\bf 
Root causes of the exploits}: We attribute all found exploits $XT_{1-9}$ to four distinct causes: 1) the presence of certain admission patterns (including $XT_1/XT_2/XT_3/XT_4/XT_6/XT_7$). For instance, $XT_4$ allows transaction replacement to cause latent overdrafts in place of valid transactions. 2) the absence of certain admission patterns to cause mempool locking (including $XT_9$ and $XT_8$). For instance, the cause of $XT_8$ on Reth is that Reth mempool is a FIFO queue, and it disallows transaction eviction of any kind, which is risky.
3) Inconsistency across multiple admission patterns, notably $XT_7$. In $XT_7$, the cause is that a mempool allows an eviction and its reversed eviction at the same time.
4) Evadable conditions to context-sensitive admission patterns, including $XT_3$ and $XT_6$. Both exploits work on Geth, where the mempool triggers the limit of transactions per send under an evadable condition (when the mempool stores more than $py_3'=5120$ pending transactions).


\noindent{\bf 
Mitigation}: We propose schemes to mitigate all newly discovered exploits comprehensively. In principle, given an exploit under a known cause, our mitigation design is to negate the cause. For instance, to mitigate $XT_4$, we propose declining transaction replacements that cause latent overdrafts. We have implemented this mitigation strategy on Geth, which was merged into the release of Geth $v1.11.4$~\cite{me:gethfix11} . Similarly, to mitigate $XT_7$, we propose ensuring the consistency between eviction events and reversed events (e.g., if admitting $tx_1$ by evicting $tx_2$ is allowed, then admitting $tx_2$ by evicting $tx_1$ is not allowed). $XT_1/XT_2$ are mitigated by disallowing eviction of valid transactions by future/latent-overdraft transactions. $XT_3/XT_6$ are mitigated by removing the triggering condition of transaction sender limit (i.e., making $py_3'=0$). $XT_8$ can be mitigated by re-enabling transaction evictions in certain cases, such as price-based transaction eviction (i.e., a pending transaction arriving later and of higher price can evict another pending transaction of lower price and admitted earlier).

If an exploit relies on multiple causes (e.g., $XT_3$  on Causes 1 and 4), negating one cause suffices to mitigate the exploit.

There are more sophisticated cases where one exploit relies on the presence of an admission pattern, and another exploit relies on the absence of the pattern. For instance, $XT_5$ relies on the presence of an admission policy named $SAP_5$ (detail in Appendix~\ref{appdx:sec:mitigate}) that turns child transactions into future ones (as in Geth), and the success of $XT_9$ relies on the absence of the same policy, that is, $\neg{} SAP_5$ (as in OpenEthereum). 
%In practice, Geth enables the policy and is vulnerable under $XT_5$, and OpenEthereum mempool disables the policy (and another policy) is vulnerable under $XT_9$.

To mitigate both $XT_5$ and $XT_9$, we propose a defense strategy in which the admission decision regarding $SAP_5$ is non-deterministic or randomized so that $SAP$ is not always on or off, making it hard for either $XT_5$ or $XT_9$ to always succeed.

We present a more formal analysis of the root causes and formal description of mitigation schemes in Appendix~\ref{appdx:sec:mitigate}.
} 

\noindent{\bf Responsible bug disclosure}: 
We have disclosed the discovered ADAMS vulnerabilities to the Ethereum Foundation, which oversees the bug bounty program across major Ethereum clients, including Geth, Besu, Nethermind, and Erigon. 

{
We also reported the found bugs to the developers of Reth, Flashbot, EigenPhi, bloXroute, BSC, Ethereum Classic and Fantom. Besides $7$ DETER bugs that \textsc{mpfuzz} rediscovered, $24$ newly discovered ADAMS bugs are reported. As of March 2024, $15$ bugs are confirmed: $XT_1$ (Nethermind, EigenPhi builder), $XT_2$ (EigenPhi builder), $XT_3$ (EigenPhi builder), $XT_4$ (Geth, Erigon, Nethermind, Besu, EigenPhi builder), $XT_5$ (Geth), $XT_6$ (Geth, Flashbot Builder, EigenPhi builder), $XT_7$ (Nethermind), and $XT_8$ (Reth).} 
After our reporting, $XT_4$/$XT_7$/$XT_8$ have been fixed on Geth $v1.11.4$/Nethermind $v1.21.0$/Reth $v0.1.0-alpha.6$. Bug reporting is documented~\cite{me:mpfuzz:report}. 

\noindent{\bf Ethical concerns}: 
When evaluating attacks, we only mounted attacks on the testnet and did so with minimal impacts on the tested network. For instance, our attack lasts a short period of time, say no more than $4$ blocks produced. We did not test our attack on the Ethereum mainnet.
When reporting bugs, we disclose to the developers the mitigation design tradeoff and the risk of fixing one attacks by enabling other attacks (described above). To prevent introducing new bugs, we did not suggest fixes against turning-based locking ($XT_5$ and $XT_6$) and locking ($XT_8$).

\vspace{-0.1in} \section{Conclusion and Future Works}
\vspace{-0.1in}
\noindent{\bf Conclusion}: This paper presents \textsc{mpfuzz}, the first mempool fuzzer to find asymmetric DoS bugs by exploring symbolized mempool states and optimistically estimating the promisingness of an intermediate state in reaching bug oracles. Running \textsc{mpfuzz} on popular Ethereum clients discovers new mempool-DoS vulnerabilities, which exhibit various sophisticated patterns, including stealthy mempool eviction and mempool locking. 

{  
\noindent{\bf Limitations and future works}: The exploit generation in this work is not fully automated. Manual tasks include mempool reduction, \textsc{mpfuzz} setup (configuring $\epsilon$ and symbols), exploit extension, etc. Automating these tasks is the future work.

\textsc{mpfuzz}'s bug oracles neither captures complete dependencies among concrete transactions nor guarantees completeness in finding vulnerabilities. Certified mempool security with completeness is also an open problem.

\textsc{mpfuzz} targets a victim mempool of limited size: the vulnerabilities found in this work are related to transaction eviction, which does not occur in a mempool of infinite capacity. Thus, the \textsc{mpfuzz} workflow cannot find exploits in the mempool of infinite capacity. It is an open problem whether a mempool of large or infinite capacity has DoS vulnerabilities. 
}


\ignore{
{{\vspace{-0.1in} \section{Discussion}
At present, the transaction symbolization of \textsc{mpfuzz} is designed by a heuristic method. Through generating one concrete transaction in each symbol, \textsc{mpfuzz} covers all the input space of transactions and the state of mempool. By prioritizing the seed with the energy designed by the heuristic method, \textsc{mpfuzz} triggers the bug oracle efficiently. A more practical method is to automatically extract the symbolized transactions by statically analyzing the control flow code path. In the control flow graph of the mempool source code, each unique code path is triggered by a group of concrete transactions. The key idea is to map each group of concrete transactions triggering the same code path into a distinct symbol. It is sufficient to cover all the code paths in mempool source code. However, whether it covers all the state of mempool needs to be studied in future. In addition, how to generate the concrete transaction by analyzing the code path as well as assigning energy score needs to be explored in the future.
}}
%\yw{Add: add a discussion section}
}

\clearpage



==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table*}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

Table with diagbox

\begin{tabular}{|c|c|}
    \hline
    alghreaiog & bghsah \\
    \hline
    cagja & \notableentry \\
    \hline
    \cellcolor{blue} & edkhaklgjaj \\
    \hline
\end{tabular}

\begin{tabular}{|p{4cm}|p{3cm}|}
    \hline
    alghreaiog & bghsah \\
    \hline
    cagja\par bla & \notableentry \\
    \hline
    \cellcolor{blue} & edkhaklgjaj \par xyz \\
    \hline
\end{tabular}

Table line/cell/column colored

\begin{table}[ht]
\centering
\begin{tabular}{c|ccccccc}
\hline
& col1 & col2 & col3 & col4 & col5 & col6 & col7 \\
\hline
\rowcolor{LightCyan}
row1& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row2& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\rowcolor{LightCyan}
row3& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row4& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\rowcolor{LightCyan}
row5& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row6& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\hline
\end{tabular}
\end{table}

\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table}[ht]
\centering
\begin{tabular}{c|g|c|g|c|g|c|g}
\hline
&col1 &col2 &col3 &col4 & col5 &col6 &col7\\
\hline
row1& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row2& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row3& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row4& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row5& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
row6& \ra & \ra & \ra & \ra & \ra & \ra & \ra \\
\hline
\end{tabular}
\end{table}



\subsection{figures}
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5.eps}
\caption{Wrapped figure}
\label{fig:perf}
\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2.eps}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10.eps}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
    ...
    *Bitmap bm = BitmapFactory.decodeFile(file)*;
    return bm;
}

void EditPicture(Bitmap bm) {
    //heavy computational picture editing
    int i = 10 (* $*$ *); //escape to plot * literatelly instead of bolden text
    bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
    for(every pixel) {
      ...
    }  
    
    //embed location information into picture
    (* $*$*)Location loc = getLastKnownLocation(Provider)*;
    (* $*$*)double longitude = loc.getLongitude()*;
    (* $*$*)double latitude = loc.getLatitude()*;
    (* $*$*)EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}
\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}
\end{center}



\subsection{misc}
\begin{itemize}
  \item cmark $\cmark$ and xmark $\xmark$
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

